Concurrent and Adaptive Extreme Scale Binding Free Energy Calculations

The efficacy of drug treatments depends on how tightly small molecules bind to their target proteins. The rapid and accurate quantification of the strength of these interactions (as measured by binding affinity) is a grand challenge of computational chemistry, surmounting which could revolutionize drug design and provide the platform for patient-specific medicine. Recent evidence suggests that molecular dynamics (MD) can achieve useful predictive accuracy (< 1 kcal/mol). For this predictive accuracy to impact clinical decision making, binding free energy computational campaigns must provide results rapidly and without loss of accuracy. This demands advances in algorithms, scalable software systems, and efficient utilization of supercomputing resources. We introduce a framework called HTBAC, designed to support accurate and scalable drug binding affinity calculations, while marshaling large simulation campaigns. We show that HTBAC supports the specification and execution of free-energy protocols at scale. This paper makes three main contributions: (1) shows the importance of adaptive execution for ensemble-based free energy protocols to improve binding affinity accuracy; (2) presents and characterizes HTBAC -- a software system that enables the scalable and adaptive execution of binding affinity protocols at scale; and (3) for a widely used free-energy protocol (TIES), shows improvements in the accuracy of simulations for a fixed amount of resource, or reduced resource consumption for a fixed accuracy as a consequence of adaptive execution.

==> adaptive-drug-discovery.tex <==
Over the last ten years a plethora of molecular dynamics simulation engines, like NAMD, Gromacs, Amber, OpenMM and more have emerged, usually specializing in a certain domain of the biologically relevant simulations field. Nonetheless all of these have been used in one form or another as the simulation engine of choice in drug discovery studies. Desmond, Amber, HTMD for example are actively used in industry to provide a complete drug discovery pipeline for pharmaceutical companies. 

The drug discovery pipeline is a well understood process that is continuously evolving, morphing from a fully experimental procedure, to more and more computational heavy, with some parts of the process already being replaced, or tested using biophysical simulation methods. In its most simple form, the aim of a drug discovery campaign is to optimize the binding affinity to a \emph{certain} target (usually a protein) as a function of a drug molecule. It aims to find the optimal drug molecule that maximizes the binding affinity (which loosely speaking is proportional to the efficacy of the medication). 

\section{Binding affinity protocols}

We have at our disposal two types of binding affinity protocols: absolute and relative. Absolute free energy methods calculate the binding affinity of a \emph{single} drug molecule to a protein, while relative methods calculate the \emph{difference} in binding affinity between two (usually similar in structure) drug molecules. The computational requirements of the two protocols differ sometimes significantly, but deciding which one is more appropriate for the task at hand is not trivial, as it is a function of resources, required time to convergence, accuracy thresholds etc.

\textbf{Introduce and describe ESMACS and TIES, with science and computational details as well.}

\subsection{ESMACS}

\subsection{TIES}

\section{Adaptivity}

Most of the aforementioned simulation engines work by way of a simple static scheme: the user hand writes a configuration file, and together with the system description (topology, PDB) it passes these files to a binary executable and waits for the simulation to be over to analyze the results. There is a disconnect between the simulation run and the user, i.e. the user has no influence over the simulation \emph{after} it has been submitted. Certain decisions, like number of time steps to run for have to be made a priory, therefore the continuous accumulation of results can, by definition, have no effect of these parameters.

% The High Throughput binding affinity calculator (HTBAC) aims to solve this problem, by abstracting the configuration files into Python objects that are customizable. It also offers an execution layer, that is able to handle a wide range of supercomputer architectures, queuing systems, etc. The performance of HTBAC has been extensively tested, with weak and strong scaling results shown in the Results sections, scaling up to XXXXX cores. 

Having the mobility and dynamism that HTBAC offers, we are able to alter our current protocols to enhance them using adaptive schemes. Utilizing adaptivity results in faster convergence rate, and more accurate results.

In the protocols section we described TIES, a relative alchemical free energy method developed by Bhati et. al. It calculate the binding affinity along an alchemical path, starting from a thermodynamics state corresponding to drug A with $\lambda=0$ ending at drug B with $\lambda=1$. The transformation from A to B is done by running simulations with different values of $\lambda$ in  the range $[0, 1]$. The original TIES protocol devised these values to be $0.0, 0.05, 0.1, ... 0.9, 0.95, 1.0$, in the hope that these intermediate values will be sufficient to correctly describe the underlying function $f(\lambda)=XXX$. Here we describe and adaptive protocol based on adaptive quadrature implemented in HTBAC, that optimally finds the correct lambda spacing of the alchemical transformation.

\subsection{Adaptive quadrature}

Description, science behind it, results in different section.

\subsection{Adaptive termination}

Time series analysis, replicas, etc.

\subsection{Adaptive protocol}

\section{System description}

The scientific and or computational improvements require validation across a number of ligand and protein complexes. We selected 3 proteins and 5 ligand pairs to run the adaptive relative free energy calculations. The systems were previously used for non-adaptive simulations by \cite{} et. al., offering a baseline comparison against our results. 

The selected proteins are the Protein tyrosine phosphatase 1B (PTP1B), the Induced myeloid leukemia cell differentiation protein (MC1) and tyrosine kinase 2 (TYK2). The five ligand pairs complexed with the proteins were taken from \cite{} study.

All systems were prepared using our automated building tool BAC \cite{} with the Amber force field for the protein, General Amber Force field for the ligands, and TIP3P water model. The complex was solvated in an orthorhombic water box with at least 14 \AA extension (systems containing around 40 thousand atoms).  

 

==> notes.tex <==
\textbf{Start with importance of binding free energy for drug design}

Binding free energy calculations rely on the physics-based molecular simulations 
and statistical mechanisms in order to predict structure-based drug design. 
Based on recent improvements in the accuracy of binding free energy, free energy 
calculations are now becoming reliable methods in the drug discovery pipeline. 
These improvements can be attributed to many advances in methodologies, as well 
as enhancements in high performance computing (HPC). Specifically, ensemble-based 
binding free energy calculations, which favor multiple shorter simulation 
trajectories over few longer simulations are showing improvements in biological 
time scales and are producing higher throughput of molecular dynamics.
These improvements can now leverage binding affinity calculations to provide 
meaningful clinical insight into computational drug campaigns and potentially 
reduce the cost of expensive experimental screening programs. 
These approaches could also be used to determine the influence of individual 
patients genetic sequence on drug efficacy in the context of clinical decision 
support. In order for these approaches to gain traction, requires using 
simulation protocols which have well-defined uncertainty and consistently 
produce statistically meaningful results. 

\textbf{2 prominent free energy protocols} 

Computational drug campaigns rely on rapid screening of thousands of compounds. 
At the start of a drug design campaign an initial screening of candidate 
compounds is conducted to filter out the worst binders before using more 
sensitive methods to refine the structure. Two prominent ensemble-based 
free energy protocols, ESMACS and TIES~\cite{Bhati2017} have demonstrated the 
ability to filter and refine the drug design process. The ESMACS (enhanced 
sampling of molecular dynamics with approximation of continuum solvent) protocol 
provides an ``approximate'' endpoint method used to screen out poor binders. The 
TIES protocol (thermodynamic integration with enhanced sampling) uses a more 
rigorous ``alchemical" thermodynamic integration approach. These protocols have 
demonstrated statistically meaningful results at timescales relevant for 
industrial computational drug campaign. 

\textbf{Scalable computing approaches that try to utilize CPU hours and cores}

Scalable simulation computing approaches such as ensemble-based free energy 
protocols in drug campaigns are utilizing the growing number of compute 
resources by scaling the number of highly parallel simulations. Most of these 
computational approaches focus on the utilization of core hours using 
fire-and-forget executions, but not many try to use core-hours effectively. 

\textbf{...But not many approaches try to use core-hours effectively}

To address the rapidly growing screening process of production scale drug 
campaigns which require screening of millions of compounds, tools that only 
leverage the scalable computation of varied binding free energy calculations on 
HPC resources are not enough to deliver on timescales that are clinically 
warranted. 

\textbf{In order to do so requires advances in methods and resource efficiency}

Moreover, free energy binding protocols need better sophistication to 
maximize resources for simulations that yield the best accuracy and precision 
given set of resources or fixed computing time. However, computational drug 
campaigns screen for compounds that are unique in chemical properties. The main 
challenge lies in the variability of statistical uncertainty of the free energy 
binding between compounds. Ensemble-based free energy protocols leverage 
generality of chemical properties to maintain convergence of binding free energy 
across compounds with variable degrees of freedom, but at the cost of 
inefficiency in resources consumption. Moreover, generality also means that 
once accuracy thresholds are reached, the protocol has converged, which prevents
protocols from achieving better accuracy for certain compounds. \jdnote{needs a 
stronger motivation} One of the 
difficulties involved in defining adequate protocols is that differences in 
drug candidate chemistry (or protein sequence) can alter simulation behavior and 
the convergence of binding strength estimates. For example, not all changes 
induced in protein shape or behavior are local to the drug binding site and, in 
some cases, simulation protocols will need to adjust to account for complex 
interactions between drugs and their targets within individual studies. Advances 
in methodologies can provide the ability to capture complexities in simulations 
for a given compound, however these methodologies rely on learning the positions 
of simulations during execution.\jdnote{alternatively we could include this 
instead of the last sentence of this paragraph: A more strategic concern is that 
during a study the requirements may change.} 
 

\textbf{Specific adaptive methods within binding free energy can enhance 
clinical insight}

Here we show how adaptive approaches within ensemble-based free energy 
protocols are designed to capture unique chemical properties and thereby 
customize the simulations for a candidate in a way that makes the most 
effective use of computational resources in order to deliver better fidelity of 
statistical uncertainties than general approaches. For drug campaigns, we can 
leverage adaptive approaches to support drug campaigns for clinical insight. 

\textbf{Suggest solution to address execution of scalable adaptive methods}

\jdnote{following paragraphs are taken from EnTK, will need to fix}
Most tools do not support the ability to encode and execute more complex 
algorithm logic, let alone provision runtime capabilities that can change 
resource configurations based on intermediately generated data.  
We need a tool that can leverage scalable execution of adaptive algorithms.

Implementation of adaptive algorithms on high performance clusters are 
predicated on adaptive runtime systems that provide the ability to make 
runtime decisions based on intermediate results and can manage resources 
efficiently. To achieve scalability and efficiency, such adaptivity cannot be 
performed via user intervention and hence automation of the control logic and 
execution is important. HTBAC enables the scalable execution of adaptive 
algorithms. 


% Leveraging ensemble-based simulations, we can now explore new adaptive sampling 
% schemes can improve sampling quality of ligand binding affinity of individual drug candidates

% \textbf{Different adaptivity schemas exist, highlight intra-protocol adaptivity but other forms of adaptivity exist}

This paper makes the following contributions:
\begin{itemize}
  \item Identifies the challenge in advancing adaptive algorithms and 
  methodologies
  \item Shows the importance of using adaptive approaches within ensemble-based
  free energy protocols to improve binding affinity accuracy given a fixed 
  amount of computing
  \item Provides the adaptive software solution (HTBAC) that enables the 
  scalable execution of adaptive algorithms
  \item Demonstrates the capability to execute adaptive applications at scale 
  and validates the scientific results from these applications.
\end{itemize}

\textbf{results of scaling experiments and intra-protocol adaptivity experiments}

This paper is organized as follows: 
Section~\ref{sec:science-drivers} describes ESMACS and TIES as ensemble-based 
free energy protocols as well as an adaptive methodology that is implemented 
within the protocol that motivates the need for higher precision given limited 
resources. 
Section~\ref{sec:related-work} describes the motivation for ensemble-based 
approaches and existing solutions and their limitations in their ability to 
support adaptive methods.  
Section~\ref{sec:htbac} describes the design and implementation of 
HTBAC--the software tool that addresses the requirements of scalable, 
adaptive methods. 
In Section~\ref{sec:experiments} we demonstrate experiments of scalability, 
validation of results, and adaptive simulation methods. We show that given a 
fixed amount of computing resources, we can achieve better accuracy and hence 
better time to solution using adaptive simulation methods. 







==> old_experiments.tex <==
Computational campaigns for drug discovery require sizable compute resources
both in terms of scale and allocation. Typically, a computational campaign
explores a large number of drug candidates by running several workflows
multiple times, each requiring thousands of concurrent simulations. Before
embarking on a drug campaign that will utilize 150 million core hours on NCSA
Blue Waters, we perform experiments to characterize the weak and strong
scaling performance of HTBAC and its overheads on Blue Waters. We validate
the results of the free energy calculations produced using HTBAC by comparing
them to results that are already available in referenced literature.

Given that protocols like TIES are more computationally demanding than
protocols like ESMACS, it is paramount to use resource efficiently,
especially for campaigns that have a predefined computational budget. As
described in Sections~\ref{sec:science-drivers} and~\ref{sec:htbac}, adaptive
simulation methods have the potential for higher computational efficiency
when compared to non-adaptive simulation methods. Specifically, adaptive
simulation methods can reduce the number of simulations for each lead
candidate without a loss in free energy accuracy and with a lower
computational load. Further, given a defined number of resources, adaptive
methods can also increase computational efficiency by improving the rate of
statistical convergence and thereby reducing the time to solution.

Specifying, coordinating and executing adaptive simulation methods requires
middleware supporting runtime decisions. As seen in Section~\ref{sec:htbac},
HTBAC has been designed to enable decisions based on intermediate runtime
results. These results are evaluated to determine a redistribution of
resource to better support the execution of new simulations. We use HTBAC to
perform experiments about adaptivity, comparing and characterizing resource
efficiency with non-adaptive simulation methods.

% - Weak Scalability Design : Keep Pipeline of Ensembles to show barrier
%   needed in S5 and S6.
% - Performance, generality with weak scaling (agnostic to kernel) Added
%   functionality (do not speak about binding adaptivity to performance or
%   generality).
% - In use case: add in why TIES is challenging, and why adaptivity is
%   challenging.

% \mtnote{General note. \\
%         - Currently, this section is a merge of two distinct contributions.
%           These need to be better merged. For example, we should consider
%           whether (i) the description of the adaptive experiments should be
%           moved to the first subsection ``Experimental Setup''; (ii) Table 1
%           should be extended to include the adaptive/nonadaptive properties;
%           (iii) the discussion of the results should have a uniform
%           argumentative format; etc.\\
%         - The structure of the section should be revise making the division
%           in subsections consistent and changing/refining their naming.\\
%         - A.0,1,2 require major rewriting of the text and the writing of
%           relevant portions of new text. This includes: (i) eliminating
%           redundant (copied) text; (ii) Eliminating or referencing text
%           copied from other publications; (iii) reorganize the argumentation
%           following the other general note left in the comments and better
%           separating the experimental variables (especially including
%           adaptive/nonadaptive) properties; (iv) adding plots (even if with
%           incomplete results) and writing an actual analysis of the results
%           for each plot.}


% \jdnote{Revisions: \\ 
%         - Rewrote experimental setup by starting with motivation and
%           explaining overview of experiments
%         - Appended all experiments to table
%         - Created subsections for weak scaling, strong scaling, validation,
%           adaptive experiments
%         - Added plots (some are incomplete) and rearranged analysis
%         - Kristof added his data for adaptive experiments and
%           wrote results 
%         - Strong scaling subsection still waiting on data from ESMACS
%         - For now, removed anything related to Titan}

% \jdnote{should we mention anything about exascale?}\mtnote{I would not but
% I would quantify the scale at which we need to run. As it stands, this
% sentence appears too generic too me.} \jdnote{mentioned lower bound on
% concurrent number of simulations}

% \mtnote{what does this mean? We cited the results already in the paper?
% These results are published?}
% \mtnote{This sentence does not read well to me. I would refine, depending
% on the answer to the previous comment}.
% \jdnote{I meant to say we validate our free energy calculation results from
% this paper with known results . Does it make more sense now?}

% \mtnote{Grammar: more than?}\jdnote{more than ESMACS}
% \mtnote{Methods for? Maybe `simulation methods'?}

% \mtnote{simulation?}
% \mtnote{simulation?} 
 
% \mtnote{Note: experiments are not adaptive, they are about adaptive
% simulation methods. Analogously, experiments are not compared to
% non-adaptive experiments but they (should) offer comparable data about both
% types of methods.} \mtnote{Note: I rewrote the whole paragraph. The
% previous version was compressed and ``left too much in the authors'
% pens''.}

% ---------------------------------------------------------------------------
\subsection{Experiment Setup}\label{ssec:exp_design}

Table~\ref{tab:experiments} shows 7 experiments we designed to characterize
the behavior of HTBAC on Blue Waters. Each experiment executes the ESMACS
and/or TIES protocol for different physical systems. Experiments 1--5 use the
BRD4 physical systems provided by GlaxoSmithKline, while experiments 6 and 7
utilize the PTP1B, MC1, and TYK2 physical systems which are a diverse set of
proteins.

\begin{table*}
    \caption{Parameters of scalability and adaptivity experiments.}
    \label{tab:experiments}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l            % Experiment ID
                    l            % experiment type
                    l            % physical system 
    %                l            % CI
                    l            % protocol type
                    l            % number of protocols
                    l            % total cores
                    }
    %
    \toprule
    %
    \B{ID}                            &  % Experiment ID
    \B{Type of Experiment}            &  % experiment type
    \B{Physical System(s)}            &  % physical system
    % \B{Computing Infrastructure (CI)} &  % CI
    \B{Protocol(s)}                   &  % protocol type
    \B{No. Protocol(s)}               &  % number of protocols
    \B{Total Cores}                   \\ % total cores
    %
    \midrule
    %
    \B{1}                             &  % Experiment ID
    Weak scaling                      &  % experiment type
    BRD4                              &  % physical system
    % Blue Waters                       &  % CI
    ESMACS                            &  % protocol type
    (2, 4, 8, 16)                     &  % number of protocols
    1600, 3200, 6400                  \\ % total cores
    % 
    \B{2}                             &  % Experiment ID
    Weak scaling                      &  % experiment type
    BRD4                              &  % physical system
    % Blue Waters                       &  % CI
    TIES                              &  % protocol type
    (2, 4, 8)                         &  % number of protocols
    4160, 8320, 16640                 \\ % total cores
    %
    \B{3}                             &  % Experiment ID
    Weak scaling                      &  % experiment type
    BRD4                              &  % physical system
    % Blue Waters                       &  % CI
    ESMACS + TIES                     &  % protocol type
    (2, 4, 8)                         &  % number of protocols
    5280, 10560, 21120                \\ % total cores
    %
    \B{4}                             &  % Experiment ID
    Strong scaling                    &  % experiment type
    BRD4                              &  % physical system
    % Blue Waters                       &  % CI
    TIES                              &  % protocol type
    (8, 8, 8)                         &  % number of protocols
    16640, 8320, 4160                 \\ % total cores
    %
    \B{5}                             &  % Experiment ID
    Strong scaling                    &  % experiment type
    BRD4                              &  % physical system
    % Blue Waters                       &. % CI
    ESMACS                            &  % protocol type
    (16, 16, 16)                      &  % number of protocols
    6400, 3200, 1600                  \\ % total cores
    %
    \B{6}                             &  % Experiment ID
    Non-adaptivity                    &  % experiment type
    PTP1B, MC1, TYK2                  &  % physical system
    % Blue Waters                       &  % CI
    TIES                              &  % protocol type
    (1, 1, 1)                         &  % number of protocols
    2080, 2080, 2080                  \\ % total cores
    %
    \B{7}                             &  % Experiment ID
    Adaptivity                        &  % experiment type
    PTP1B, MC1, TYK2                  &  % physical system
    % Blue Waters                       &  % CI
    TIES                              &  % protocol type
    (1, 1, 1)                         &  % number of protocols
    2080, 2080, 2080                  \\ % total cores
    %
    \bottomrule
    %
    \end{tabular}
    }
\up{}
\end{table*}

Experiment 1 and 2 measure the weak scalability of HTBAC using multiple
instances of the ESMACS (experiment 1) and TIES (experiment 2) protocol.
Experiments 3 uses both the TIES and ESMACS protocols, characterizing the
weak scaling of heterogeneous protocol executions. Experiments 4 and 5
measure the strong scalability of HTBAC using a fix number of instances of
the ESMACS (experiment 4) or TIES (experiment 5) protocol. Experiments 6 and
7 characterize nonadaptive and adaptive simulation methods using the TIES
protocol.

In each weak scaling experiment (1--3), we keep the ratio between resources
allocated and protocol instances constant. Consistently, for each experiment
we progressively increase both the number of cores (i.e., measure of
resource) and the number of protocol instances by a factor of 2. In each
strong scaling experiment (4--5), we change the ratio between resources
allocated and the number of protocol instances. For each experiment, we fix
the number of protocol instances and reduce the number of cores by a factor
of 2.

Weak scaling experiments provide insight into the size of the workload that
can be executed in a given amount of time, while strong scaling experiments
show how the time duration of the workload scales when adding resources. For
all the weak and strong scaling experiments we characterize the overheads of
HTBAC, EnTK and RP, and we show an approximation of the time taken by the
resources to become available. This offers insight about the impact of HTBAC
and its middleware on the time to completion of each workload.

For weak and strong scaling experiments, we reduced the number of time-steps
of the protocols and omitted the analysis steps $S5$ and $S6$ of their
workflows (Figure~\ref{fig:ties_esmacs_application}). These simplifications
are consistent with characterizing scalability performance instead of
simulation duration. For the experiments 1--5 we used the following
time-steps: $S1=1000$; $S2=5000$; $S3=5000$; and $S4=50000$.

Experiments 6 and 7 compare the the accuracy and time to solution of
nonadaptive and adaptive simulation methods. For the nonadaptive simulation
method of Experiment 6 we use 13 preassigned and approximated $\lambda$
windows, consistent with the value reported in Ref.~\cite{Bhati2017}. In this
way, we produce 65 concurrent simulations for stages $S1$--$S4$ of the TIES
workflow (Figure~\ref{fig:ties_esmacs_application}). The production
simulation stage $S4$ executes each simulation for 4ns. Stage $S5$ consists
of 5 analysis tasks which aggregate the simulation results of $S4$. The
global analysis stage $S6$ contains a single task that aggregates the results
from $S5$.

In the adaptive workflow~\ref{fig:adaptive_ties}, we initialize the TIES
protocol with 3 $\lambda$ windows, obtaining 15 replicas. We separate stage
$S4$ of each TIES replica into 4 sub-stages. Each sub-stage runs a 1ns
simulation, followed by an adaptive quadratures analysis which estimates free
energy errors with respect to each interval of two $\lambda$ values. We
evaluate the total number of $\lambda$ windows as determined by the adaptive
quadrature results in order to measure the differences in time duration
between adaptive and non-adaptive methods as well as the differences in
accuracy.

% \mtnote{I had to simply this paragraph a lot. Please check whether I
% omitted some essential detail or got the algorithm wrong.}
% \jdnote{it works}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/Adaptive_TIES.pdf}
  \caption{Adaptive workflow for TIES. After equilibrating 3 initial
  $\lambda$, the first production stage starts. This is followed by analysis
  at every $\lambda$ interval, to decide whether to add a new window in
  between. In our implementation, the production-analysis cycle is repeated
  for 4 production steps, not shown here.}
\label{fig:adaptive_TIES}
\end{figure}

% \mtnote{For quality reasons, it would be better to use figures in pdf
%   format.}\jdnote{addressed}.

For Experiment 6, we assigned the following simulation time-steps: $S1=3000$;
$S2=50000$; $S3=50000$; and $S4=2000000$. The adaptive simulation method of
Experiment 7 uses the same simulation time-steps, apart from $S4$ which is
divided into 4 sub-stages of 500000 time-steps each. 

% \jdnote{should we
% mention relationship between ns and time-steps?}

We performed all the experiments on Blue Waters, a 26868 node Cray XE6/XK6
SuperComputer with peak performance of 13.3 petaFLOPS managed by NCSA. We
initiated the experiments from a virtual machine outside NCSA. In this way,
we did not run any persistent process on the NCSA login node, consistent with
NCSA usage policies. We used HTBAC 0.1, EnTK 0.6, and RP 0.47 and the same
versions of the \texttt{NAMD-MPI} MD kernel, compiled according to the
capabilities of each environment and of \texttt{NAMD} itself, and launched
via the \texttt{aprun} command. For the analysis stages in the TIES protocol
we used \texttt{AmberTools}.

NCSA sets a system policy on the maximum number of processes that
\texttt{aprun} can spawn, limiting the number of concurrent tasks we can
execute on Blue Waters to approximately 450. During the execution of
Experiment 2, we observed failing tasks once we scale up to 8 TIES protocol
instances, which is equivalent to 520 concurrent tasks. In a trial of 10
repetitions at this scale, we observed an average of 70 failing tasks, with a
standard deviation of 6.67, and range of 59 to 83 tasks. Given that we only
ran a small number of trials, more data would be required to properly model
the distribution type of these results.

NCSA allows to run only one MPI application for each compute node. As a
consequence, we had to run each MD simulation with 32 cores (i.e., one full
compute node) even if our performance measurement of \texttt{NAMD} on Blue
Waters indicated that 16 cores would offer the best trade-off between
computing time and communication overhead.

% \jdnote{Should we include the scalability plot of
% a single NAMD task using aprun?}

% \mtnote{The following paragraphs are disconnected from the previous ones.
% We need a `joining' paragraph starting from something like: ``We designed n
% experiments\ldots We used m protocols\ldots See Table o\ldots''. Moved a
% paragraph here as a starting point.}\jdnote{provided ``segway"}

% Experiment 2 measures weak scaling performance of ESMACS at higher scales,
% using ORNL Titan.
% \mtnote{Would it be better to describe weak scaling in terms of solution
% time, number of resources and problem size, as done in the following
% paragraph?}\jdnote{moved to previous para when first introducing weak
% scaling}

% of the protocols \mtnote{which protocols? So far we wrote about methods
% (but we did not specify what type of methods are we referring to)}
% \jdnote{Does the modified description of the protocol types in the earlier
% paragraph give enough insight?} \mtnote{required by what/whom? ``keeping
% the number of pipelines fixed at the number required by \ldots'' or
% something like that?} \jdnote{I've changed this description of ws, do this
% sentence and the next suffice?}

% By design of each protocol, an increase in the number of instances means an
% increase in the number of pipelines. Further, \jdnote{mention the
% relationship between protocols and pipelines in section IV.}

% \mtnote{property of? I would replace with: ``weak scaling provides
% insight\ldots''} provides insight

% Next, we measure strong scaling performance of the ESMACS and TIES
% protocols in experiments 4 and 5, respectively, by fixing the number of
% protocol instances, but reducing the cores by a factor of 2 in each run.

% \mtnote{which ones?} by fixing the workload i.e. \mtnote{Grammar: please be
% careful about the use of `i.e.' as explained in my previous set of
% comments}
% \mtnote{Why do we need the `i.e.' at all? What does `workload' add?
% ``\ldots by fixing the number of pipelines of each protocol and reducing
% \ldots''}
% \jdnote{also changed this description of ss.}

% the number of cores by a factor of 2 in each run.

% \mtnote{what does `timing' mean in this context? Duration? }
% \jdnote{will be defined in section IV}\mtnote{we will define
% `what'?}\jdnote{ignore earlier comment, the correct phrasing is time
% duration of the workload, but I am not sure if this causes
% confusion}\jdnote{ also workload will be defined in Section IV}

% \jdnote{expecting linear speedup, and expect fixed overheads}\mtnote{is
% this comment about text that still needs to be written? If so, I would not
% mention expectations of results in the design section.}

% \mtnote{of?}\jdnote{addressed}

% Experiments 4 measures the strong scaling performance of ESMACS while
% experiment 5 repeats the same strong scaling experiment using the TIES
% protocol.

% \mtnote{This is a placeholder for an actual paragraph: note how the
% previous paragraphs have a structure based on numbering experiments (and
% referring them to the table via references that are still missing), while
% this and the following paragraphs do not use the same structure. Please
% expand as needed and note that a section is not `ready' until this kind of
% uniformity is not achieved.}\jdnote{I've added experimental design of
% adaptive/nonadaptive methods.}

% Keep iterating on the next two paragraphs to get the right description from
% Kristof

% We perform the experiments for the nonadaptive (experiment 6) and adaptive
% (experiment 7) simulation methods with the same number of cores and
% simulation duration (Table~\ref{tab:experiments}). By fixing these
% parameters, we enable the comparison between the accuracy and time to
% solution of the two methods.

% By design of the nonadaptive TIES workflow
% (Figure~\ref{fig:ties_esmacs_application}), each $\lambda$ window creates a
% new simulation condition that must be replicated. TIES requires 5 replicas
% per $\lambda$, thereby producing $\lambda \times 5$ or simulations.

% \mtnote{Reference table and exp number}
% \jdnote{addressed in this and previous sentence}
% \mtnote{Reference table with S*}
% \jdnote{the ref to Figure~\ref{fig:ties_esmacs_application} already points
% to the description of S*, no?}
% \mtnote{Grammar: no spaces before and after dashes}
% \jdnote{noted}
% \jdnote{reworded this paragraph}

% \mtnote{Grammar: it is not clear to what this `this' refers to} produces a
% total of 65 concurrent simulations for stages $S1$--$S4$ \mtnote{Reference
% table with S*} \mtnote{Grammar: no spaces before and after
% dashes}\jdnote{noted}. The production simulation stage $S4$ executes each
% simulation for 4ns. The analysis stage $S5$ assigns 5 analysis tasks which
% aggregate simulation results of $S4$ with respect to each replica. The
% global analysis stage $S6$ contains a single task that aggregates the
% results from $S5$.

% \mtnote{different from what?}\jdnote{changed}

% The estimation of the error determines whether
% \mtnote{Grammar: as already commented in the previous draft, `whether'
% implies already `or not'.\jdnote{noted} Adding it is
% redundant.}\jdnote{noted} to spawn additional $\lambda$ windows. If the
% error estimate in a certain interval is higher than the acceptable
% threshold, a new $\lambda$ window is assigned halfway between the interval.
% If the critical threshold is reached, we have reached convergence and the
% application stops; else, current simulations continue executing and new
% simulations begin executing based on newly generated $\lambda$ windows.

% The estimation computation \mtnote{This is too compressed. In itself,
% `estimation computation' means little. The reader has to go back to the
% previous paragraph to understand what those two words refer to. `We compute
% the free energy errors\ldots'?} is captured \mtnote{`captured' is
% metaphorical. Metaphors should be avoided when writing science. Also, the
% sentence is passive and also this should be avoided in scientific writing}
% as a single stage \mtnote{Does the reader know what a stage is?} containing
% a single task. By design of the adaptive quadrature algorithm \mtnote{where
% this algorithm is used? Does the reader know about it?}, the number of
% additional $\lambda$ windows will vary across candidates, which will impact
% the number of simulation-analysis iterations. \mtnote{And\ldots We are
% missing an explanation of why this is important from an experimental design
% point of view. Maybe because it changes the number of tasks?}
% \jdnote{will call this something else}.\jdnote{check with Kristof on the
% local and global analysis that happen for nonadaptive}

% \mtnote{Note: paragraphs like this indicate lack of iteration before
% releasing the manuscript for review. Too much is assumed, too little is
% converted from thoughts to written form. How the academic writing process
% works: Before releasing the manuscript for review, the author goes back and
% forth across the manuscript multiple times. Progressively, each paragraph
% is iterated until it is grammatically correct and it stands on its own
% content-wise. When a manuscript is received for review, the reviewer focus
% on the content of each paragraph and section, assessing their completeness
% and conceptual/formal correctness. Each grammatical error, each
% inconsistency or missing detail distracts the reviewer impeding her
% work.}\jdnote{I've removed the previous paragraph that gave trouble and
% updated the experimental setup of the adaptive and non-adaptive methods.}

% This procedure is repeated until convergence, at which point all concurrent
% simulation are terminated. We define convergence as the point in the
% production-analysis loop at which a desired error threshold is reached.

% When one protocol has converged whilst another has not, we can shift
% computational resources to favor simulations that require additional
% resources.

% individual\mtnote{I am not sure I understand what individual means in this
% context}

% strong scaling performance of ESMACS and TIES on Blue Waters. We fix the
% number of protocols and vary the amount of resources in order to produce
% generations

% \mtnote{The reader will struggle to understand what `generations' means in
% this context.} of execution.
% \mtnote{Two sizable paragraphs to describe weak scaling, four lines to
% describe strong scaling? I would expand.}

% \mtnote{This sentence seems to suggest that we run our experiments on a
% virtual machine. I know what you mean but the average reader has no idea
% about the capabilities of our middleware and the policies of not executing
% persistent processes on the head node of Blue Waters.}
% \jdnote{Can we omit this sentence?}

% and the Titan ones from an ORNL login node. as Blue Waters does not permit
% executing applications directly on the login node. The ORNL Titan
% experiments had instead to be performed from an ORNL login node.

% The minimization tasks of $S1$ to 1000 simulation time steps, while the
% equilibration tasks in $S2$ and $S3$ are \mtnote{Grammar: inconsistent
% tense. `Were' or `assign'} assigned 5000. The MD simulation tasks in $S4$
% are assigned 50,000 steps.

% \mtnote{when/why a simulation task is `production'? I am not sure I
% understand what that means}\jdnote{removed production for weak/strong.
% Production applies to adaptive/nonadaptive which need to show the
% production scale timesteps i.e. 2 or 3M}

% while on Titan a non-MPI, multi-core NAMD engine. On Titan we compiled NAMD
% with CUDA for the ESMACS experiments, and with OpenMP for the for TIES ones
% as NAMD does not support alchemical perturbations execution on GPU.

% application launch method, which is the NCSA Blue Waters designated command
% for describing the application parameters and resource requirements
% \mtnote{does the reader know what is a launch method?} \jdnote{better?}
% \mtnote{Unfortunately not: https://bluewaters.ncsa.illinois.edu/using-aprun
% . Alternative: `We perform (or performed depending on what tense you will
% decide to use) all Blue Waters experiments using the \texttt{aprun} command
% to launch the MD simulations'}.
% \jdnote{noted and addressed.} During our scalability experiments we found
% two main limitations.
% \mtnote{this is too generic. Based on this paragraph, we found two main
% limitations. This is what we should therefore write.}

% \jdnote{I've changed this again because the limitation on the max no. of
% concurrent CUs is a system setting (similar to what we experienced
% first-hand on Titan), but it's not a technical limitation of APRUN.}

% Unfortunately, \texttt{aprun} has several \mtnote{this is too generic.
% Based on this paragraph, we found two main limitations. This is what we
% should therefore write.} limitations: First, the number of concurrent tasks
% execution is limited to \ldots. On average, during our experiments we were
% not able to execute more than 436 concurrent tasks.
% \mtnote{how do we know this average?}.
% \jdnote{would it make sense to show a bell curve of the distribution of
% failing units? I have 8 data points, but I can run more and include Mark's
% Cray paper?}
% \mtnote{Agreed. The comment was about saying that you observed this average
% while performing experiments. See how I rewrote the paragraph}.
% \jdnote{added the data for the failing units however including a
% distribution of this data is not meaningful as the sample size in the
% number of trials is very small. By looking at some histograms where I vary
% the bin size, it could be either Gaussian or multimodal distribution. Only
% more data will tell us for sure what kind of distribution we have.
% Moreover, Mark's Cray paper shows range of concurrent units using ORTE-LIB,
% so I will not reference this here.}

% \mtnote{this is metaphorical. Please change using a factual predicate.}
% \jdnote{changed the phrasing a bit}
% \mtnote{Note: I had to rewrite the paragraph because the current version
% was too unrefined. Please see the note above about the need to
% progressively refine each paragraph.}

% From our own scalability performance measurements of NAMD on Blue Waters,
% we observe the ideal cores per task to be 16, however Blue Waters does not
% permit running multiple MPI applications on the same node, hence each NAMD
% task requires a complete node to maintain concurrency.
% \mtnote{This needs to go before previous sentence as it explains why we use
% 32 cores for each NAMD executable. Note: it is not true that NAMD
% `requires' 32 cores as stated above.}\jdnote{moved here since this para
% discusses \texttt{aprun} limitations}

% In order to continue execution on higher scales \mtnote{Why do we need an
% higher scale?}, we perform higher scales \mtnote{I am not sure what
% `performing higher scales' means} on ORNL Titan, using the ORTE launch
% method \mtnote{Why don't we use ORTE on BW? The reader will probably know
% that they are similar machines}.

% The difference in platforms produces overheads \mtnote{Only overheads or
% also different execution time of NAMD---seeing the differences described in
% the previous paragraph} that can be captured by RTS \mtnote{does the reader
% know what a RTS is?} and are shown \mtnote{careful with the use of
% `demonstrate', especially in a scientific paper} in the figures
% \mtnote{which figures?} as "APRUN overhead" and "ORTE overhead"
% \mtnote{LaTeX requires different quotes}.

% For tasks pertaining to $S1$ -- $S4$ \mtnote{What are $S1$ and $S4$? LaTeX
% wants double dash without space to indicate a range}, while the analysis
% stage, $S5$ use AmberTools \mtnote{grammar: I am not able to parse this
% sentence}.

% For both adaptive and nonadaptive experiments \mtnote{the reader knows
% about Experiment 1-7, not about adaptive/nonadaptive ones},

% In the nonadaptive experiments,

% For the adaptive experiments, each substage
% \mtnote{What is a `substage'?} of $S4$ i.e. $S4.1$--$S4.4$ is assigned
% 50,000 steps.\mtnote{Why the difference is number of steps and why it is
% relevant?}

% HTBAC submits a resource request to EnTK, to which EnTK uses RP to acquire
% resources via a single pilot. Accordingly, we request the maximum number of
% cores required by the workload as the number of cores in a pilot.

% To characterize the weak scaling performance of TIES \mtnote{I am not sure
% I understand this sentence: For measuring the weak scaling performance of
% TIES?}
% \jdnote{better?}, we use between 4160 and 33280 cores as indicated in
% Figure~\ref{fig:weak_scaling_TIES} because the NAMD executable used in all
% tasks \mtnote{does the reader know what a task is in this context?}
% \jdnote{will be defined in Section IV} from $S1$-$S4$ require
% \mtnote{grammar: requires} a single node i.e. 32 cores per task, as
% mentioned earlier in the APRUN limitation.
% \mtnote{why?}\jdnote{32 cores/task addressed by earlier mention of aprun
% MPI limit}

% For strong scaling performance, we fix the number of protocol instances to
% 8 instances given that we experience failing concurrency of tasks when we
% scale the workload to 8 protocols.\mtnote{why 8?} We vary the amount of
% resources as shown in Figure~\ref{fig:strong_scaling_TIES} by showing
% reducing of resources by a factor of 2. \mtnote{Please expand indicating
% and justifying the the chosen amount of resources. Experiments can be
% design in many ways, we need not only to describe but also to justify why
% we choose a specific design for our experiments.}\jdnote{better?}

% For the TIES protocol, each pipeline \mtnote{does the reader know what a
% pipeline is?}\jdnote{will be address in Section IV} consists of six stages
% \mtnote{simulation stages?}. Each of the simulation stages contains a task
% for every unique ($\lambda$, replica) combination \mtnote{does the reader
% understand this?}\jdnote{will be addressed better in section IV}. In the
% non-adaptive workflow \mtnote{we never used `workflow'. Previously we used
% non-adaptive (written as `nonadaptive') experiment. Note that we did not
% introduce adaptive/nonadaptive experiments} scenario, the first 11
% $\lambda$ windows
% \mtnote{does the reader know what a lambda window is?} consist of the
% following values: $L$ is a vector with
% \begin{flalign} L &= \{ x_i: x_i\in[0,1]\; and\; x_{i+1} = x_i + \delta \},
% where\ \delta\ is\ 0.1. %&$$L=\{ x_i: x_i\in[0,1]\; and\; x_{i+1} = x_i +
% \delta \}$$%, where $\delta$ is $0.1$.
% \end{flalign}

% We append two additional values on both ends of $L$, completing 13
% $\lambda$ windows. Each $\lambda$ window consists of five replicas.
% Therefore there are a total of 65 tasks for every simulation stage
% \mtnote{depending on the previous sections of the paper, this `therefore'
% may have to be better explained to the reader}. The production simulations
% stage, $S4$ as described in figure~\ref{fig:pst}\mtnote{missing figure}
% executes a 4 ns simulation duration \mtnote{grammar: executes a simulation
% for 4 ns? a simulation with a 4 ns duration?}. The analysis stages of the
% protocol reduce the number of tasks \mtnote{Why/how?}. The first analysis
% task consists of five tasks where each task performs an aggregate analysis
% over all $\lambda$ windows for each replica. The second analysis stage
% consists of one task that aggregates the previous results and computes a
% single average across all replicas.

%----------------------------------------------------------------------------

\subsection{Characterization of Scalability Experiments}

\mtnote{I would create a subsection with overheads, discussing their behavior
and nature while referencing both weak and strong scaling experiments.}
\jdnote{placing this here...}

We perform 5 experiments to characterize the overheads of HTBAC, EnTK and the 
runtime system, and \texttt{aprun} as a function of weak and strong scaling 
properties. We compare these overheads to the total execution time of all the 
tasks to assess their overall impact on the application duration. 
The durations we measure are defined as:

\begin{itemize}
    \item \textbf{Task Execution Time}: Time taken by the task executables to 
    run on the CI. 
    \item \textbf{HTBAC Overhead}: Time taken to process the application, instantiate the 
    components and subcomponents, translate protocols into pipelines for EnTK, 
    and validate resource descriptions. 
    \item \textbf{EnTK and RP Overhead}: Time taken by ensemble management system and the 
    runtime system to submit and manage the execution of tasks. 
    \item \textbf{\texttt{aprun} Overhead}: Time taken by \texttt{aprun} to schedule
    tasks on a set of compute nodes. 
\end{itemize} 

Total Time to Execution \(TTX\) measures only the aggregated execution time of 
all tasks' executables. 
\mtnote{TTX should measure only the aggregated time spent executing the
tasks' executables. All the rest should be part of RP overhead} 
\jdnote{
This sentence doesn't need to go in but I wanted to clarify a point: I would 
like to know if we should use TTX as TTX or something else like Task Execution Time. 
We have TTX measured by events: \texttt{cu-exec-start} and \texttt{cu-exec-stop}
, since \texttt{aprun} doesn't allow further scrutiny using events like 
\texttt{app-start} until \texttt{app-stop}. 
We use the term TTX internally, but maybe for this paper we should call it task 
execution time. TTX sounds like time to execution which could interpret the 
entire application, no?}

Once the runtime system relinquishes control flow to \texttt{aprun}, the 
precise times of when \texttt{aprun} schedules the task on the compute
nodes and when the MD kernel begins execution cannot be measured. Instead we 
approximate the \texttt{aprun} overhead by measuring the difference between 
TTX/Task Execution Duration and the total \texttt{NAMD} execution time, provided
by the \texttt{NAMD} output logs. 

% We characterize the execution time of all three applications \mtnote{which one?},
% \jdnote{given that I mention what each experiment entails earlier, can I keep 
% the application general and say all 3?} and overheads of HTBAC, EnTK, RP and 
% \texttt{aprun}. 

% \jdnote{Since we are showing overhead component separate, can we remove the
% total overhead calculation?}

% The total time to completion (TTC) of each application \mtnote{of what?} 
% \jdnote{per application} \mtnote{you see the difference produced by my 
% editing?} can be expressed as $TTC = TTX + T_{O}$ where Total Time to Execution 
% \(TTX\) measures only the aggregated execution time of all tasks' executables. 
% \mtnote{TTX should measure only the aggregated time spent executing the
% tasks' executables. All the rest should be part of RP overhead}\jdnote{for
% discussion with Matteo 06/04}\mtnote{I am afraid I do not understand this
% comment} 




% % $T_{O}$ equates to the total overheads produced by HTBAC, EnTK, and
% % RP: $$T_{O} = T_{O}\textsuperscript{HTBAC} + T_{O}\textsuperscript{EnTK} +
% % T_{O}\textsuperscript{RP}$$ 




% \mtnote{As defined, this formula seems to add
% twice part of the RP overheads.}
% \jdnote{I think I'm missing something: The RP
% overhead is what I get from the pilot duration logs. Not sure where I'm
% duplicating}
% % \mtnote{If TTX is more than just the aggregated execution time of
% % all the tasks' executable, then TTX and $T_{O}$ both contain part of RP
% % overhead.}

\subsection{Weak Scaling and Performance Characterization}\label{ssec:ws}

% \mtnote{Is this meant to be a subsubsection?}\jdnote{changed weak, strong
% and adaptive experiments \& results to subsections}

We investigate the weak scaling of HTBAC using three
applications \mtnote{which ones?}\jdnote{addressed}: Experiment 
1 using TIES-only, Experiment 2 using ESMACS-only, and Experiment 3 using
both TIES and ESMACS configurations. Each application uses a different protocol 
configuration with a number of instances determined by the 
number of concurrent executions supported by \texttt{aprun}. In each experiment, 
we increase the number of instances of the protocol configuration, 
proportionally to the amount of requested resources. 

Experiment 1 in Figure~\ref{fig:ws} (a) measures the weak scalability of HTBAC 
with the TIES protocol. Each instance of the TIES protocol contains a single 
pipeline with 4 stages and 65 concurrent tasks. We increase the number of 
instances linearly, between 2 and 8. When scaling to 8 protocol instances, we 
execute beyond the average limit of 450 concurrent tasks. 
Nevertheless, we include results at this scale to show HTBAC's performance 
capabilities in supporting higher orders of concurrent simulations. 

Experiment 2 in Figure~\ref{fig:ws} (b) measures weak scalability with the 
ESMACS protocol. We increase the number of instances linearly, between 2 and 16. 
Each ESMACS protocol contains 1 pipeline with 4 stages and 25
concurrent tasks \mtnote{Do we `increase the number of instances linearly,
between 2 and 8' also in experiment 2? If so, we should say that only once
for Experiment 1--3. If not, why?}\jdnote{addressed the scaling ranges, and 
explained why}. 

Experiment 3 in Figure~\ref{fig:ws} (c) measures weak scalability
with instances of both TIES and ESMACS protocols. Also in this case, we scale
the instances of both protocols linearly, between 2 and 8. The first 
configuration shows 1 ESMACS and 1 TIES protocol, and with each increase in 
scale we double the number of protocols. Experiments 2 and 3 
show scalability ranges within the limit of the maximum number of concurrent 
tasks we can successfully execute on Blue Waters. For all weak
scaling experiments we use \mtnote{Grammar: conjugation}\jdnote{back to the 
present} physical systems from the \texttt{BRD4-GSK} library with the same 
number of atoms and similar chemical properties. The uniformity of these 
physical systems ensures a consistent workload that is insignificant to any 
variability in performance characterization. 
\jdnote{this is to say that the fluctuations in
execution times between data points are invariant to the physical
systems}\mtnote{Nice comment, I would edit it and put it in the text!}.
\jdnote{addressed}

% \mtnote{does the reader know what a task is in this context?} \jdnote{will
% be defined in Section IV}



% \mtnote{grammar: I do not understand the sentence after the `;'} given by
% the sum of the constituent overheads: $$T_{O} =
% T_{O}\textsuperscript{HTBAC} + T_{O}\textsuperscript{EnTK} +
% T_{O}\textsuperscript{RP}$$.


\dwwnote{The figure captions and legends don't appear to agree which axis 
applies to which measurement. Also the legend should be inside the plots.}
\jdnote{addressed, except with subplots I figured it would look cleaner with the
legend at the bottom.}

\begin{figure}
  \centering
    \includegraphics[width=\columnwidth]{figures/ws_all.pdf}
    \caption{Weak scaling properties of HTBAC. We
    investigate the weak scaling of HTBAC as the ratio of the number of
    protocol instances to resources is kept constant. Overheads of HTBAC, 
    EnTK + RP, and \texttt{aprun}, and Task Execution Time as a function of (a)
    TIES protocol (Experiment 1), (b) ESMACS protocol (Experiment 2) , and (c) 
    TIES and ESMACS protocols (Experiment 3). We ran 3 trials for each 
    experiment.} 
\label{fig:ws}
\end{figure}

\jdnote{Maybe combine captions into 1?}\mtnote{Agreed.}\jdnote{One figure, 3 
subplots, 1 caption is cleaner}

In all weak scaling experiments (Figure~\ref{fig:ws}) we
observe Task Execution Time to be fixed as the number of protocol increases, 
thereby showing ideal weak scaling behavior. \mtnote{Please refine the previous 
sentence as it might not say what I think you want to say: What does it mean 
that TTX is `within error margin'? And how this relates to `ideal weak scaling 
behavior'? Maybe the former applies to the latter instead of TTX?}.
\jdnote{does this read better?} The error bars are calculated
using 3 trials per protocol instance measure. While it is highly desirable to use 
larger trials to determine the precision of our observations, our current data
already suggests a trend of reproducibility. \mtnote{This might be consider
little without further explanation}\jdnote{how is this?}

The HTBAC overhead depends mostly on the number of protocol instances that
need to be generated for an application. This overhead shows a super linear
increase as we grow the number of protocol instances, but its duration is
negligible when compared to Task Execution Time.

Furthermore, an additional overhead, driven by the \texttt{aprun} launch
method increases as we approach a system limit on the number of concurrent
\texttt{aprun} processes. For example, when scaling to 8 TIES protocol
instances as shown in Figure~\ref{fig:ws} (a), we account for
additional time that is factored into Task Execution Time. The increase in 
\texttt{aprun} overhead occurs when tasks show failure which introduces 
additional communication between the nodes that run the job (i.e. MOM Nodes) and 
an attempt to relaunch failed tasks.  
\mtnote{We need to explain why TTX is affected. Are tasks restarted?
Also, does this overhead matter? See previous comment about RP overhead
impact on TTX/TTC/Resource utilization.}\jdnote{added a technical detail}

% HTBAC enables concurrent execution of multiple protocol \mtnote{what type
% of protocols?} instances.

The runtime overheads, mainly EnTK and RP, mostly depend on the number of
tasks that need to be translated in-memory from a Python object to a
task description~\cite{dakka2017}. For RP this is confirmed in 
Ref.~\cite{merzky2018} 
\mtnote{This sentence is copied from
a previous paper we wrote: does the reader know what a CU is?}
\jdnote{I will add in a brief mention of CU in Section IV}\mtnote{I would
just use task as you do in the following sentence. IMHO, using CU adds yet
another pseudo-technical term as a synonym of a term we are already using,
i.e., task}\jdnote{noted and added reference for RP as well}.
As such, those overheads are expected to grow proportionally to
the number of tasks as observed in Figure~\ref{fig:ws} (a)--(c), bars in 
blue color.
\mtnote{Please add reference to the relevant figure(s) and details.} 
\jdnote{addressed}
The RP overhead is calculated measuring and aggregating the execution time
(i.e., duration) of the RP components that manage and coordinate the
execution of the application. Among these components, the task scheduler of
RP introduces the largest overhead. The task scheduling overhead scales
linearly with the number of tasks because the time taken to schedule a task
depends on the total number of tasks that need to be scheduled. 

\mtnote{I commented all the following. IMHO, it does not contribute to
understand the current analysis of the results. Do we need to expand the
analysis?}\jdnote{It can be left out, I was just trying to explain the barriers
in EnTK between stages that may incur on the overheads, given that all 
simulations need to finish before moving on to next stage. With protocols that
have more tasks/stage, I thought this should be mentioned as a contribution.}
% ------------------------- COMMENTED BY MT -------------------------
% EnTK submits CU descriptions to a database that is then pulled by
% RP.\mtnote{I am not sure this is accurate}\jdnote{took out "same" database}
% In addition, each stage constructed by EnTK maintains sequential barriers.
% \mtnote{Doe the reader know what a barrier is?}\jdnote{I will add this to
% the EnTK description in Section IV} RP remains dormant until completion of
% the current tasks before staging the next tasks. \mtnote{This figure is
% about scaling behavior, not about the mechanics of EnTK and RP here
% discussed.}\jdnote{took out figure ref}
% ------------------------- END COMMENTED BY MT ----------------------

% The impact of the synchronization barriers increases with the number of CUs
% as seen in the 16 protocol instances data point in
% This pull operation occurs over a wide area networks, which introduces
% varying amounts of latency.


In comparison to Task Execution Time, the EnTK and RP overheads are 
an order of magnitude shorter, yet contribute directly to the total duration of 
the application. Ultimately, in a computational drug campaign, the use of 
runtime systems results in additional allocation of resources. In situations where
campaigns are limited by a computational budget, we approximate those overheads 
would contribute to $\approx15\%$, based on the data in Figure~\ref{fig:ws}.
For such campaigns, efficient utilization of resources is most crucial 
consideration. In the scope of this work, we leverage the efficiency of 
resources as provided by the runtime system, in order to focus on scalable 
execution of adaptive methods that can improve accuracy and reduce time to 
solution. \mtnote{I am afraid this whole paragraph needed to be
rewritten. I tried to fix it but we are missing a comparative evaluation of
this overhead. For example, does this overhead matter when compared to TTX or
TTC? Given a computation campaign with TIES and ESMACS, how much allocation
time would be spent on this overhead? What would be the total percentage of
allocation/resources spent in overheads?}\jdnote{added context}

% The main contributor to the increase in overhead in RP is based on the the
% time of resources inactivity while RP schedules new tasks. As such, the
% overhead is expected to grow proportionally to the number of concurrent
% tasks~\cite{dakka2017}.


% Among these durations, the pilot duration contains the time to bootstrap
% and terminate the pilot. The task overheads contain the executor's spawning
% of the task, folder staging preparation, and operating system task
% spawning. \mtnote{We need to explain to the reader why all this is relevant
% in this context.} \jdnote{need to discuss on 06/04, should we keep these
% details or keep the focus on the paragraph just above this one?}



% \mtnote{this sentence does not read well. I would refine it}
% \mtnote{this needs further explanation}
% \jdnote{reworded paragraph, also commented out next paragraph on EnTK
% synchronization until I can justify better.}

% \mtnote{Does the reader know what aprun is? Also, I would use something
% like textttt to identify the name of a command or
% executable}\jdnote{addressed}

% \mtnote{concurrent?}\jdnote{addressed} 

% Together, the EnTK-enabled synchronization barriers and \texttt{aprun}
% overhead failures \mtnote{until now, we have implicitly assumed that our
% overheads are measured in time. Did we now use also number of failures?}
% introduce delays in the scheduling of the CUs and results in higher
% overheads \mtnote{Is this sentence circular? Overhead increases
% contributing to increasing the overhead?}. Lastly, we notice that each
% additional protocol instance contributes to roughly 55 additional seconds
% in \(TTX\).\mtnote{All this needs to be clarified and expanded into an
% actual discussion of the results.}

% We use between 4160 and 16,640 cores as indicated in
% Figure~\ref{fig:weak_scaling_TIES}.

% To characterize the weak scaling performance of TIES \mtnote{I am not sure
% I understand this sentence: For measuring the weak scaling performance of
% TIES?}
% \jdnote{better?}, we use between 4160 and 33280 cores as indicated in
% Figure~\ref{fig:weak_scaling_TIES} because the NAMD executable used in all
% tasks \mtnote{does the reader know what a task is in this context?}
% \jdnote{will be defined in Section IV} from $S1$ -- $S4$ require
% \mtnote{grammar: requires} a single node i.e. 32 cores per task, as
% mentioned earlier in the APRUN limitation.
% \mtnote{why?}\jdnote{32 cores/task addressed by earlier mention of aprun
% MPI limit}

% With each new protocol instance generated for an application, the HTBAC
% overhead grows to match the additional requirement of generating new
% protocols.

% In order to understand the contribution of the various events in HTBAC,
% termed as HTBAC overhead, to

%----------------------------------------------------------------------------
% \subsubsection{Weak Scaling Experiments}

% We investigated the weak scalability properties for the TIES protocol by
% growing the number of protocol instances while adhering to the required
% number of pipelines. By design of each protocol, an increase in the number
% of instances simply means an increase in the number of pipelines. The first
% weak scalability experiment demonstrates the behavior of HTBAC, EnTK and RP
% using the multiple instances of the TIES protocol. By design of weak
% scaling, the ratio between the number of pipelines and cores are kept
% constant. As the number of cores (measure of resource) changes by a factor
% of 2, we introduce twice as many protocol instances. As designed, the weak
% scaling property provides insight into the size of the workload that can be
% investigated in a given amount of time.\mtnote{This paragraph is a copy of
% a previous paragraph. See comments and iterations of the previous paragraph
% before rewriting a new paragraph if needed.}

% ---------------------------------------------------------------------------
\subsection{Strong Scaling and Performance Characterization}

\mtnote{Should we have also a `Weak Scaling Experiments' header? Or maybe we
should change this one?}
\jdnote{I changed this subheader to match the subheader
+or weak scaling \& performance characterization}

To investigate strong scaling, we run two applications on Blue Waters: strong 
scaling of TIES (experiment 4) and strong scaling of ESMACS 
(experiment 5). \mtnote{Please add name of the applications}.
\jdnote{addresed} 

We investigate the
strong scaling behavior considering only homogeneous protocols. We base this 
consideration on supporting the experiments of adaptivity in which we  
show adaptive methodology only for TIES. Experiments of strong scaling
show how the time-to-solution varies when consistently increasing the number of 
resources for a fixed problem size. We leverage strong scaling to support the 
objective in this work, which is to characterize (a) the time-to-solution 
differences between adaptive and nonadaptive methods (b) the increase in the 
number of resources as required by the nonadaptive method to reach the 
required accuracy threshold. 
\mtnote{I am afraid we will need a better explanation for this omission}.
\jdnote{
    Added context. Note about this paragraph: I think the argument about strong 
    scaling only homogeneous protocols can be reduced to the fact that we only 
    show TIES adaptivity. But for the rest of the paragraph, is there merit to 
    put some of these ideas into experiment design?}


Both applications use the \texttt{BRD4-GSK} physical
systems \mtnote{Should this detail go in experiment design? This would apply
also to the weak scaling in the previous section}.
\jdnote{It's already mentioned in design so we can omit}


% The objective of strong scaling enables us to examine the properties of 
% adaptive methods. 

% Given the adaptive and nonadaptive methods: if we run the adaptive method 
% we achieve time to solution X. With the nonadaptive method, we achieve time to 
% solution Y 

% We provide the adaptive and nonadaptive methods a fixed amount of resources: 

% The nonadaptive method runs in time Y with Z accuracy 
% The adaptive method runs in time X with N accuracy

Experiment 4 \mtnote{name?}\jdnote{addressed} shows the strong scaling behavior 
of TIES alone \mtnote{Are you sure this should not be the `nth experiment shows'}
, using \texttt{NAMD-MPI} with 32
cores per task. We fix the number of instances of the TIES protocol to 8 due
to the described \texttt{aprun} limitations. We vary the amount of resources
between 4160, 8320 and 16640 cores. Given 4160 cores, we can execute 4
generations of 130 concurrent tasks; with 8320 cores, we can execute 2
generations of 260 concurrent tasks. Experiment 5 shows the strong scaling 
behavior of the ESMACS protocol \mtnote{See previous comment about
application/experiment}\jdnote{fixed}. We fix the number of instances of the 
ESMACS protocols to 16 and vary the amount of resources between 3200, 6400 and 
12800 cores. This produces the same number of generations of execution 
\mtnote{add reference to the subsection where generation is defined} as shown in 
experiment 4. We define generations of execution in Section~\ref{ssec:exp_design}. 

In Figure~\ref{fig:ss}, we observe linear speedup in Task Execution Time for
both experiments with increase in number of cores. The availability of more 
resources for a fixed number of protocols explains this behavior. 

All overheads remain constant for both experiments when increasing the number 
of cores. The scheduling the number of tasks as opposed to the amount of 
resources, is the main driver of the fixed runtime overheads, namely EnTK and 
RP. This is confirmed for RP in Ref.~\cite{merzky2018}.


% The comparison between weak and strong scalability shows the overhead
% introduced by load balancing and scheduling tasks in multiple generations.

% By design of the TIES protocol, this workload show up to $65 \times 8$
% concurrent tasks, where each task uses 32 cores. The total number of
% concurrent

% \mtnote{See previous comments about terminology}\mtnote{I am not sure I
% understand: are we comparing overheads when weak and strong scaling our
% applications/workflows or are we first measuring the overheads when strong
% scaling and then comparing them to those of weak scaling?}. As we scale the
% number of generation of concurrent tasks executions, we half the resources
% allocated by the pilot \mtnote{this should be explained in the experiment
% setup and design}.

\mtnote{General note. Experiments about weak and strong scaling show the
behavior of our software stack with one or more workflows/workloads. The
question these experiments answer to is: Given a workload/workflow, does this
software stack scale weakly and/or strongly? This is why, in the analysis of
our data, we look at the linearity (or lack of thereof) of our plots. The
analysis of the overhead(s) answer to a different question: What part of a
measure---e.g., time to completion---depends on the properties of an element
used to produce that measure---e.g., a component of our software stack?
Usually, the analysis of the overheads is used to explain why we observe lack
of scalability (weak or strong) as represented by a superlinearity in our
plots. The discussion of our experimental results should clearly distinguish
these questions and properly relate the study of scalability to that of
overheads. At the moment, our discussion does not do all this.}\jdnote{I
reduced the discussion of scalability down to the properties that relate to
contributions of overheads and trends observed in TTX.}

\begin{figure}
  \centering
   \includegraphics[width=\columnwidth]{figures/ss_all.pdf} 
   \caption{Strong scaling properties of HTBAC. We investigate the strong 
    scaling of HTBAC by fixing the number of protocol instance and increasing 
    the number of cores. Overheads of HTBAC, EnTK + RP and \texttt{aprun}, and
    Task Execution Time as a function of (a) TIES protocol (Experiment 4) and
    ESMACS protocol (Experiment 5). We ran 3 trials for each experiment.}
\label{fig:ss}
\end{figure}


%----------------------------------------------------------------------------
\subsection{Experiments Validation}

% HTBAC automates the process of calculating the binding affinity of
% protein-ligand complexes from reading the input to analyzing the final
% results.

In order to validate the correctness of the results produced using HTBAC and
the BRD4-GSK physical systems, we compare our results with those previously
cited \mtnote{This is unclear. Do you mean: results that have been previously
published? If so, where?}. These experiments \mtnote{What experiments? The
previous sentence writes about a comparison.} are vital to gain confidence in
the algorithm \mtnote{which algorithm?} and to prove that it is indeed
calculating the correct values.

The validation experiments were based on the original study of Wan et
al.~\cite{Wan2017brd4} \mtnote{Note: `et al.' is an abbreviation of 'et
alia', Latin for `and [et] others [alia]'. As such, the correct spelling is
`et al.'. It is now corrected both here and in the table caption}. We
selected a subset of the protein ligand systems that were the subject of that
study: ligand transformations 3 to 1, 4, and 7. We then performed a full
simulation on all 3 systems and calculated the binding affinity using HTBAC.

The results of our experiments, collected in Table~\ref{tab:exp2}, show that
all three $\Delta \Delta$G values are within error bars of the original study
using the TIES protocol, reinforcing \mtnote{validating? Based on what we
wrote before this would seem to contradict our intent} the fact that the
results produced using HTBAC are indeed correct
\mtnote{I am not sure `correct' here applies to the results. We may want to
have a look about the difference between validation and verification,
focusing on the separation between methodology and results.}.

\begin{table}
  \centering
  \caption{Comparison of the calculated binding free energies using HTBAC,
  from the original study by Wan et al. and experimental data. In
  principle,\mtnote{Do they use the same protocol? If there are differences
  we should explain them.} the two theoretical studies used the same
  protocol. This experiment proved that HTBAC implemented TIES correctly, as
  the calculated values are either the same or within error bar of the
  original study. All values are in \textbf{kcal mol\textsuperscript{-1}}.}  
  % \begin{tabular}{l@{\hskip 1in}r@{\hskip 0.2in}r@{\hskip 0.2in}r}
  \begin{tabular}{lrrr}
    \toprule
    System & HTBAC & Wan et. al & Experiment \\
    \midrule
    BRD4 \textbf{3 to 1} & \num{0.39 +- 0.10} &   \num{0.41 +- 0.04} &  \num{0.3 +- 0.09} \\
    BRD4 \textbf{3 to 4} & \num{0.02 +- 0.12} &   \num{0.01 +- 0.06} &  \num{0.0 +- 0.13} \\
    BRD4 \textbf{3 to 7} & \num{-0.88 +- 0.17} &  \num{-0.90 +- 0.08} & \num{-1.3 +- 0.11} \\
    \bottomrule
  \end{tabular}
  \label{tab:exp2}
\end{table}

%----------------------------------------------------------------------------
% \subsection{Adaptive Experiments}

% The TIES workflow can benefit from an adaptive execution environment to
% improve the efficiency and accuracy of result. In \emph{adaptive
% experiments} we implemented the adaptive quadrature algorithm specifically
% customized for biosimulations.

% In the adaptive workflow, we alter the number of $\lambda$ windows being
% simulated over the course of a protocol instance. The position of new
% $\lambda$ windows depends on the estimated error of the integral measured
% between adjacent windows. Increasing the number of $\lambda$ windows in
% regions of rapid change will increase the accuracy of the overall integral
% to a greater degree than an arbitrarily placed window. In order to
% adaptively add lambda windows, we need access to the $\partial
% U/\partial\lambda$ values during runtime. Therefore, we break down the
% single production simulation stage (S4) \mtnote{I would reference the
% figure with the workflow diagram here} from the nonadaptive workflow into
% multiple smaller stages \mtnote{how many?}, each running for 1 ns. Once
% each simulation is complete within a stage, a decision is made about
% whether more $\lambda$ windows are required, and, if so, where these
% windows should be placed.

% We start out the simulation with 5 replicas of 3 \mtnote{why emphasis for
% 3?}\jdnote{addressed} equally spaced $\lambda$ windows, and equilibrate
% them. Then we repeatedly execute shorter production simulations followed by
% an analysis phase which determines where to place new lambda windows. This
% procedure is repeated until convergence, at which point all concurrent
% simulation are terminated. We define convergence as the point in the
% production-analysis loop at which a desired error threshold is reached.

% The success of this algorithm is determined by the decision where
% additional $\lambda$ windows should be introduced. In adaptive quadrature,
% this decision is made by calculating an error estimate on the integral and
% comparing this estimate to a threshold value. Due to the stochastic nature
% of biosimulations, it is non-trivial to determine this error and, as a
% proof of concept, we simplified this decision to replicate pre-calculated
% results. In future studies, we plan to use a dynamic decision process.

% Inter-node communication introduces a constraint on the number of new
% $\lambda$ windows that can be added at each iteration. Simulations must run
% on an integer number of nodes to reduce the overhead of inter-node
% communication. This means that the number of new $\lambda$ windows (i.e.,
% the number of simulations) \emph{has} to be either doubled or left
% unchanged. If the number of windows is doubled, the number of nodes per
% simulation can be halved automatically. Our algorithm loops through the
% current $\lambda$ window pairs until this criterion is reached, forcefully
% adding more windows when needed.


% I don't think we need this equation here, it's too trivial.
% \begin{flalign} L &= \{ x_i: x_i\in[0,1]\; and\; x_{i+1} = x_i + \delta \},
% where\ \delta\ is\ 0.5. %&$$L=\{ x_i: x_i\in[0,1]\; and\; x_{i+1} = x_i +
% \delta \}$$%, where $\delta$ is $0.1$.
% \end{flalign}

% For every $\lambda$ window we initialize with five replicas therefore
% yielding a total of 15 tasks. We run 15 tasks for stages $S1$ through
% $S4.1$. Between stages $S4.1$ and $S4.3$ the number of $\lambda$ windows
% doubles for every stage, which doubles the total number of tasks. The last
% production simulation stage, $S4.4$, runs for the remaining 2 ns durations.

% Our experiments implement adaptive change in the $\lambda$ windows sampled
% and not the timing of execution. In this way, we introduce only a single
% \mtnote{additional?} degree of freedom relative to \mtnote{compared to?}
% our baseline ``non-adaptive" experiments. HTBAC provides the functional
% capability to adaptively determine the time at which the $\lambda$ windows
% are chosen. However, in this paper we do not investigate the impact of such
% adaptivity, as the objective is to determine the feasibility of adaptive
% execution and the scientific merit of adaptive decision making.

%----------------------------------------------------------------------------


% \begin{figure}
%   \centering
%     \includegraphics[width=\columnwidth]{figures/adaptive_vs_nonadaptive_ps
%     eudo.pdf}
%     \caption{Illustrating the adaptive vs. non-adaptive workflow given the
%     same number of core hours}
% \label{fig:adaptive_vs_nonadaptive_TIES}
% \end{figure}

% ---------------------------------------------------------------------------
\subsection{Adaptive Experiments}

The lack of adaptivity in most workflows usually comes down to the way
simulation engines (like NAMD, Gromacs, Amber and others) work. The user hand
writes a configuration file, and together with the system description (topology,
PDB) it passes these files to a binary executable and waits for the simulation
to be over to analyze the results. There is a disconnect between the simulation
run and the analysis, i.e. the intermediate results can have no influence over
the simulation \emph{after} it has been started. Therefore, certain decisions,
like number of time steps to run for have to be made \emph{a priori}, and the
continuous accumulation of results can, by definition, have no effect of these
parameters.

Having the mobility and dynamism that HTBAC offers, we are able to alter our
current protocols to enhance them using adaptive schemes. Utilizing adaptivity
results in faster convergence rate, and more accurate results.

The aim of introducing adaptive quadrature to alchemical free energy
calculation protocols (e.g. TIES) is to reduce time to completion while
maintaining (or increasing) the accuracy of the results. Time to completion
is measured by the number of core hours consumed by the simulations. Accuracy
is defined as the error with respect to a reference value, calculated via a
dense $\lambda$ window spacing (65 windows). This reference value is used to
establish the accuracy of the non-adaptive protocol (which has 13 $\lambda$
windows) and the adaptive protocol (which has a variable number of $\lambda$
windows, determined at run time).

One of the input parameters of the adaptive quadrature algorithm is the
desired acceptable error threshold of the estimated integral. We set this
threshold to the error of the non-adaptive algorithm calculated via the
reference value. The algorithm then tries to minimize the number of $\lambda$
windows constrained by the accuracy requirement.

Table~\ref{tab:adapquad} shows the results of running adaptive quadrature on 5
protein ligand systems, comparing the \(TTX\) and accuracy versus the
non-adaptive case. The number of lambda windows are reduced on average by
\SI{32}{\percent}, hence reducing \(TTX\) by the same amount. The error on the
adaptive results is also decreased, on average by \SI{77}{\percent}. More
importantly, the error on all of the systems are reduced to below \num{0.2}
kcal/mol, which has recently been shown \cite{} to be the upper bound of
reproducibility across different MD engines. 

The TTX of the TYK2 L7-L8 system has increased for the adaptive run by 1
$\lambda$ window compared to the non-adaptive case. This is due to the
non-adaptive error begin very low, and matching that same accuracy required the
use of a large number of windows. Nonetheless due to the efficient placing of
the windows, the accuracy of the free energy still increased by
\SI{40}{\percent}.

\begin{table*}
  \caption{Comparing results of adaptive, non-adaptive and reference runs}
  \label{tab:adapquad}
  \begin{tabular}{lSSSSSS}
    \toprule
    {System}                               & 
    {Ref $\Delta \Delta$G}                 &
    {Non-adaptive $\Delta \Delta$G}        &
    {Adaptive $\Delta \Delta$G}            &
    {Num. of $\lambda$ windows}            &
    {Decrease in time to completion}       &
    {Increase in accuracy}                 \\
    \midrule
    {PTP1B L1-L2}   & 
    -58.51 & 
    -57.87(64) & 
    -58.60(9) & 
    10 & 
    \SI{23}{\percent} & 
    \SI{86}{\percent} \\
    %
    {PTP1B L10-L12} & 
    1.83   & 
    2.05(22) & 
    1.94(7)  & 
    6  & 
    \SI{54}{\percent} &
    \SI{68}{\percent} \\
    %
    {MCL1  L32-L38} & 
    2.13   & 
    2.33(20) & 
    2.14(1)      & 
    7  & 
    \SI{46}{\percent} & 
    \SI{95}{\percent} \\
    %
    {TYK2  L4-L9}   &
    -28.69 & 
    -28.25(44) & 
    -28.67(1)  & 
    7  & 
    \SI{46}{\percent} & 
    \SI{98}{\percent} \\
    %
    {TYK2  L7-L8}   & 
    4.97   & 
    4.92(5) & 
    5.00(3)      & 
    14 &  
    \SI{-8}{\percent} & 
    \SI{40}{\percent} \\
    \bottomrule 
    
  \end{tabular}
\end{table*}

Figure~\ref{fig:adapconv} shows progression of the algorithm, starting from 3
initial lambda windows, and at each iteration bisecting the interval where the
error is above the set threshold. For system X, we can see as how the parts of
the function that change less have relatively fewer windows, while parts of
greater change (usually, though not always around the $\lambda=0.5$ mark) have
more $\lambda$ windows to represent the shape of the function more closely.

% \kfnote{Move this to algorithm description} In previous studies \cite{} the
% error estimation during the adaptive algorithm is done by calculating the
% integral estimate using two methods, one lower and one higher in complexity,
% then the difference between the two can constitute as a rough estimate of the
% error on that interval.

\begin{figure}
  \input{figures/fig-adapt.tex}
  \caption{Plot of the error estimate as a function of the resource consumption
  comparing the adaptive and nonadaptive simulations. While the error estimate
  converges for both simulations, the adaptive simulation places the lambda
  windows in such a way that the error is considerably lowered. This is a plot
  for one of the systems.}
  \label{fig:adapconv}
\end{figure}

\begin{figure}
  \input{figures/fig-savings.tex}
  \caption{Quantifying the benefits of the adaptive quadrature simulations. (a)
  The error of the adaptive run is reduced for all 5 test systems sometimes by a
  s significant amount. Recently \cite{} it has been shown that reproducibility
  of free energy calculations can be achieved up to 0.2 kcal/mol. The adaptive
  algorithm brings down the error of the non-adaptive simulations below this
  threshold, ensuring that results and also reproducible. (b) Resource
  consumption is also reduced, except for one of the systems, where the low
  error threshold required more $\lambda$ windows to fulfill.}
  \label{fig:savings}
\end{figure}

Adaptive quadrature is specific to alchemical free energy calculations.
\emph{Adaptive termination}, the second adaptive protocol implemented in HTBAC,
offers dynamic termination for any simulation protocol that has as its aim the
prediction of an observable value. The protocol monitors the convergence of the
observable as the simulation progresses, and stops the execution when a
criterion has been met. Non-adaptive protocols usually have a predefined
simulation time, set based on the assumption that the simulation will converge
by that time. This means that in practical examples the simulation might have
converged before the predefined time interval. 

In the original TIES protocol the simulation has to be run for
\SI{4}{\nano\second} and the results are analyzed thereafter. This pre assumes
that all systems need this time interval for the results to converge. In reality
certain could systems converge faster, and terminating the simulation before the
statice 4 ns end, could lead to faster time to insight and less compute
resources consumed. Adaptive termination was implemented in HTBAC by having a
checkpoint every $\tau = \SI{0.5}{\nano\second}$ in the simulation. Results show
that the adaptively terminated TIES protocol saves compute resources and reduced
time to insight on average by \SI{16}{\percent} for the physical systems we
tested.

\begin{figure}
  \input{figures/fig-term.tex}
  \caption{Adding caption soon!}
  \label{fig:termination}
\end{figure}




==> old_introduction.tex <==
...One of the defining challenges facing computational chemistry is the accurate
determination of the strength of small molecule binding to target proteins.
Reaching this goal would allow computational approaches to replace or
supplement experimental techniques in drug design and refinement pipelines.
This has the potential to reduce the cost of expensive experimental screening
programs but in order to do so requires the capability to rapidly screen
thousands of candidate compounds. Recent improvements in both simulation
algorithms and hardware exploitation mean that macromolecular binding free
energies estimated from molecular simulation are reaching accuracies that can
emulate successful drug campaigns ~\cite{DeVivo2016}.

\jhanote{this idea needs better contextualization and motivation. at a minimum
references will be needed to substantiate the claim.} Specifically, ensemble-
based approaches, which favor multiple shorter simulation trajectories over
few longer simulations, are showing improvements in biological time scales.

% Most advances in high-performance computing have focused on the scale,
% performance and optimization of single long simulations. Due to the end of
% Dennard scaling, methodological advances and resource architectures (in 
% particular GPGPUs), many applications are now formulated using multiple, shorter 
% ensemble-based simulations. 

\jhanote{It is unclear what "these developments" are} These developments are resulting in
higher throughput of molecular dynamics and thereby increasing industrial
interest. Furthermore, the same technologies which are applicable in drug
discovery could also be used to determine the influence of individual patients
genetic sequence on drug efficacy in the context of clinical decision support.
In order for these approaches to gain traction however, requires the
development of simulation protocols which have well-defined uncertainty
\jhanote{uncertainty in what?} and produce statistically meaningful results.
This continues to represent a significant computational challenge. \jhanote{In
previous paragraph, it is unclear what "technology" is being referred to, and
what  "approaches" are being referred to.}

One of the difficulties involved in defining adequate protocols is that
differences in drug candidate chemistry (or protein sequence) can alter
simulation behavior and the convergence of binding strength estimates. For
example, not all changes induced in protein shape or behavior are local to the
drug binding site and, in some cases, simulation protocols will need to adjust
to account for complex interactions between drugs and their targets within
individual studies. A more strategic concern is that during a study the
requirements may change. \jhanote{Is a study, a set of simulatixons? a specific
simulation? A campaign?}

A typical example of this is that at the start of a drug design campaign
an initial screening of candidate compounds is conducted to filter out the worst 
binders before using more sensitive methods to refine the structure.

% <<<<<<< HEAD Moreover, the "fire and forget" mentality no longer fulfills
% computational efficiency when campaigns are limited by a computational
% budget or require timely insight for clinical efficacy.
% =======

These complexities of protocol selection and refinement can be captured using 
adaptive algorithms, where task  dependencies are not known 
\textit{a priori} and are predicated on intermediate results. 
\jhanote{This is a definition of an adaptive workload, not an adaptive
application or adaptive algorithm. Most people who develop applications and
algorithms don't think in terms of task graphs!}

\jhanote{Why is this in the introduction and not related / background work?}
In bio-simulations, several classes of adaptive algorithms exist which tackle
different problem spaces. For example, an increasingly popular approach is to
used Markov state models (MSM)to learn a simplified representation of the
phase space explored by simulations and use this to inform which regions are
further sampled in future simulations (cite).

Successful drug campaigns require adaptive algorithms in order to increase 
the fidelity of statistical uncertainty and thereby reduce time to convergence 
for a drug candidate. \jhanote{Is the purpose of the following to motivate
new adaptive sampling algorithms?}
Leveraging ensemble-based simulations, we can now explore 
new adaptive sampling schemes which increase convergence and improve 
sampling quality of ligand binding affinity of individual drug 
candidates~\cite{DeFabritiis2014}. 
\jhanote{Why is this in the introduction and not related / background work?}
Other adaptive methods such as replica exchange and well-known variations of
replica exchange i.e. replica exchange with solute tempering (REST) use the
Metropolis-Hastings criteria to make periodic decisions that impact which
regions of the phase space are being sampled\jdnote{@dww which citation goes
well with this? the wang2015 paper only mentions FEP}.


\jhanote{Why is this in the introduction and not related / background work?}
Metadynamics and expanded ensemble (EE) dynamics are another class of 
adaptive algorithms, where like replica exchange, individual simulations 
can jump between simulation conditions. Once the error threshold 
criteria is met for a drug candidate, the algorithm can decide to halt 
simulations for that candidate while the next candidate is considered. 
Adaptive quadrature algorithms (cite) are a simple and attractive option for 
achieving this in so called `alchemical' free energy methods which involve 
integrating the area under a curve drawn by sampling along a transformation 
coordinate. Adding additional simulations in regions where the curve is 
changing most rapidly reduces errors on the predicated binding affinity. 
Once an uncertainty threshold criteria is met for a given candidate, the 
algorithm can decide to halt simulations for that compound while the next 
candidate is considered. This approach could even be combined with enhanced 
sampling techniques such as REST (cite). 

Until recently, simulation based studies of binding free energies have
generally been limited to at most tens of drug-target combinations. As
simulation campaigns become larger and more ambitious the inefficiency, and
associated cost, of "fire and forget" approaches based on standardized
sampling (e.g. simulations of fixed length designed to ensure some level of
convergence) are multiplied. \sout{Both limited computational budget and/or
strict time to insight deadlines are characteristic 
applications and drive the need to be able to obtain reliable results in an
optimal manner.} 
Strict bounds on time-to-solution exist for clinical insight. This requires
both scale and efficient utilization of computational resources. Adaptive
approaches are capable of reducing the computational effort and allowing
informed trade-offs between factors such as convergence tolerance, time to
completion and computational cost. \jhanote{convergence of what? i don't think
we've identified what convergence here is?}

% Most advances in high-performance computing have focused on the scale,
% performance and optimization of single long simulations. Due to the end of
% Dennard scaling, methodological advances and resource architectures (in 
% particular GPGPUs), many applications are now formulated using multiple, shorter 
% ensemble-based simulations.  
% These methods in bio-simulation science have been developed to take advantage of 
% the growing number of compute resources where multiple tasks are executed on 
% these compute resources in parallel. Although these methods may suffice for 
% existing problems, studying more drug candidates systems for longer durations 
% will require sophistication in these algorithms. 
% There are however, limited software solutions that can support the 
% scalable execution of multiple tasks concurrently.

Implementation of adaptive algorithms on high performance clusters (HPCs) are 
predicated on adaptive runtime systems that provide the ability to make runtime 
decisions based on intermediate results and can manage resources efficiently. 
\jhanote{Now focus on
HPC Challenges for Adaptivity, instead of revisiting a point that has been
made 3 times. Also, I don't know what enhancements in adaptive algorithms you
are referring to. What is the problem / limitation that we are trying to
enhance?} \sout{For molecular simulations to truly influence decision making
in industrial and clinical settings, the dual challenges of scalability of
drug candidates and enhancements in adaptive algorithms will need to be
tackled.} It is also possible that as simulation and machine learning
approaches converge higher level decisions of what simulations should be run
may also be automated, requiring adaptive runtime frameworks. There are
however, limited software solutions that can support the adaptive execution of
high throughput binding affinity calculations at scale. \jhanote{OK so there
is missing software. But what is the technical challenge or missing
capabiliteis that this software must provide? The reader is unable to discern
that so far. Also the challenges / missing capabilities must be clear before
going into a discussion of HTBAC, c.f.. paragraph which begins with
"In order to support.."}

% >>>>>>> 8e69b71820a07495000ed0c06ca7acb3baf7fd62


% Adaptive quadrature 
% algorithms (cite) deliver this requirement by adding additional simulations to 
% reduce errors on the predicated binding affinity. Once the error threshold 
% criteria is met for a candidate, the algorithm can decide to halt simulations 
% for that candidate while the next candidate is considered. 



% and other  adaptive sampling techniques guide 
% simulations toward improving sampling quality by steering execution towards more 
% interesting regions of phase space (cite). 




% Tools that facilitate the automated scalable and sophisticated computation of
% varied binding free energy calculations on high-performance computing
% resources are necessary. 

We have previously developed a tool for automating
system building and simulation input generation, the Binding Affinity
Calculator (BAC)~\cite{Sadiq2008}. More recently we have introduced the 
High-Throughput Binding Affinity Calculator (HTBAC)~\cite{dakka2017}, 
which brings advances in the design of domain-specific workflow systems 
using building blocks to facilitate the automation of deployment 
and execution of rapid binding affinities on leadership class machines. 

% These methods in bio-simulation science have been developed to take advantage of 
% the growing number of compute resources where multiple tasks are executed on 
% these compute resources in parallel. Although these methods may suffice for 
% existing problems, studying more drug candidates systems for longer durations 
% will require sophistication in these algorithms. 


% which provides a domain specific interface to leverage recent advances in
% abstracting the relatonships between building blocks in workflow systems to


% In Dakka \textit{et al.}~\cite{dakka2017} we 
% demonstrated how HTBAC scales almost perfectly to hundreds of concurrent 
% multi-stage pipelines for a single protocol. 

%, which permits rapid time-to-solution that is essentially invariant
%of the size of candidate ligands.

% as well as the type and number of protocols concurrently employed.

%In this paper we aim to reproduce a collaboration project between UCL and
%GlaxoSmithKline to study a congeneric series of drug candidates binding to the
%BRD4 protein 
%(inhibitors of which have shown promising preclinical efficacy in
%pathologies ranging from cancer to inflammation)
%~\cite{Wan2017brd4}. This
%study compared two different protocols, known as TIES and
%ESMACS~\cite{Wan2017brd4, Bhati2017}, both based on an ensemble simulation
%philosophy. 


For scalability studies, we reproduce results from a collaboration project 
between UCLand GlaxoSmithKline to study a congeneric series of drug candidates binding to
the BRD4 protein (inhibitors of which have shown promising preclinical
efficacy in pathologies ranging from cancer to
inflammation)~\cite{Wan2017brd4}. These studies employed two different
protocols, known as TIES and ESMACS~\cite{Bhati2017}, both based on multiple
simulations of the same system. 

% In this paper we reproduce results from a study of  congoneric series of
% componds which employed two different protocols, known as TIES and
% ESMACS~\cite{Wan2017brd4, Bhati2017}, both based on multiple simulations of
% the same system.

%In this approach multiple simulations are executed based on the
%same input system description, providing enhanced sampling and reduced time to
%completion. 
TIES is rigorous but computationally expensive and has a limited range of 
applicability.
ESMACS is approximate but can be employed across any set of ligands at lower 
computational cost.
%TIES is based on rigorous, but computationally expensive,
%calculations of relative free energies (i.e. results provide a comparison
%between two drugs). ESMACS, in contrast, provides absolute binding free
%energies at low computational cost, but to achieve this coarse grains many of
%the details of the system being studied. The simplifications employed by
%ESMACS can reduce its effectiveness in some systems. 
%In the real world
%application of these technologies, d
Drug design projects have limited resources,
%and must make trade-offs between the needs for rigour and coverage of a wide
%range of chemical space. 
%Initially large numbers of compounds must be screened
so initially large numbers of compounds must be cheaply screened
to eliminate poor binders (using ESMACS), 
%later 
before more accurate methods (such as
TIES) are needed as good binders are refined and improved. %This means that
%many projects will combine the use of both protocols.

%We explore the use of HTBAC for aforementioned sophisticated exploration of
%novel compounds binding to a target protein. 
In order to support such
investigations, in addition to being scalable, HTBAC must be enhanced to
support flexible resource reallocations schemes where resources can be moved
between simulations run using different protocols or systems, for example,
when one calculation has converged whilst another has not. This adaptability
makes it easier to manage complex programs where efficient use of resources
is required in order to achieve a time to completion of studies comparable to
those of high throughput chemistry. 


To demonstrate computational efficiency in adaptive approaches over nonadaptive, 
we show results of 3 proteins and 5 ligand pairs to run the adaptive relative 
free energy calculations. These systems were previously used for non-adaptive 
simulations by \cite{} et. al., offering a baseline comparison against our 
results.


% \dwwnote{Could the next sentence go?}
% This functionality provides the
% foundations upon which we develop adaptable simulation schemes that
% automatically handle different system characteristics.




% In principle, many workflow management systems (WMS) can be used to express
% ensemble-based workflows to compute binding free energies. General-purpose WMS
% are however,  limited by a lack of specificity: workflow system with feature
% rich, but complex interface models impose substantial overhead when
% integrating application workflows in the runtime system, preventing users from
% quick and flexible applications prototyping.

% Furthermore, statistically meaningful results derived from simulations are of
% critical interest, as they can leverage additional sampling of simulations
% which could lead to an improvement in precision of free energy calculations.
% Such decisions typically, cannot be made {\it a priori} and require postmortem
% user intervention in order to analyze and spawn additional simulations.
% Specific features such as steering and adaptivity (e.g., spawning additional
% simulations) during runtime often require a redistribution of resources.
% Current WMS do not provide adequate support for dynamic resource utilization
% and require special extensions for adaptive formulations thus limiting the
% possibility of adaptive workflows.


In this work we demonstrate the use of HTBAC to enable adaptive  
algorithms to optimize for computational efficiency by coordinating runs with 
% Calculations using either protocol require simulations of free and 
% protein bound ligand necessitating the coordination of runs with 
heterogeneous computational requirements.
%Executing either protocol often involves
%running simulations of both free and  bound  ligand, with the later involving
%a much larger system than the former. This means that even single calculations
%must coordinate simulations with heterogeneous computational requirements.
Further to the use of a common framework to improve the ease of deployment and
efficiency of execution of existing protocols we show how HTBAC can aid the
development of enhanced approaches. 
%We demonstrate this capacity through the development of a variant of TIES 
%employing adaptive sampling which improves time to convergence.

%The TIES protocol is highly sensitive to
%the chemical details of the compounds being studied, which means that
%different runs may require different sampling strategies to achieve optimal
%time to convergence. We have developed an adaptive variant of TIES which
%automatically increases the sampling in areas where it is needed for each
%system, allowing more rapid convergence of calculations. Furthermore, this
%approach facilitates a data driven approach to future protocol refinement.

%This approach not only allows us to tailor the protocol to the particular
%system but to provide meaningful statistical uncertainties for all of our
%models. 
These developments fit into a wider vision in which the use of
flexible and responsive computational protocols produce accurate,
precise and reproducible estimates of the free energy of binding with 
meaningful error bars. Not only would this allow for wider uptake of 
computational techniques in industrial settings but opens up possibilities 
of using these technologies in clinical decision support scenarios. By creating 
a `digital twin', where the target protein is based on the real patients 
genetic sequence, a specific individuals response to different 
treatments could be predicted. 

% \dwwnote{Could remove the next sentence}
% This approach would be
% applicable even in the case of rare variants where insufficient data is
% available for statistical methods to be informative.

\jhanote{Is this paper about HTBAC or about the methodological (not science) advances that come about using HTBAC?} 
The novel contributions of HTBAC are: (i) Unprecedented throughput: it allows
the concurrent screening for drug binding affinities of multiple compounds at
unprecedented scales, both in the number of candidates and resources utilized;
(ii) Agile selection of different binding affinity protocols
(iii) Support for adaptive algorithms, which provides the
efficient execution of individual protocols leading to resources being assigned
at runtime and maximizing computation efficiency. 

% In future, we will demonstrate
% how the above set the stage for design of experiments that will allow for
% optimization of the collective and overall time-to-insight as opposed to any
% single simple calculation.

%\dwwnote{Do we need the next paragraph? A slightly shortened version is: }

In this paper we describe the background to our binding free energy protocols
and how we designed HTBAC to meet the challenges faced in bringing this
approach up to extreme scale. We then describe a set of experiments
characterizing the performance and scalability of HTBAC and the enhancement in 
computational resources in adaptive execution. 

% In the next section, we review previous work using ensemble molecular dynamics
% and outline the challenges faced in bringing this approach up to extreme
% scale. Section 3 provides details of the TIES and ESMACS protocols and the
% BRD4 system we will apply them to. In Section 4, we discuss how HTBAC has
% been designed and implemented in order to meet the computational challenges
% associated with the scalable execution of multiple, and possibly concurrently
% executing protocols. In Sections 5 and 6 we describe the design and then
% results of a series of experiments characterizing the performance and
% scalability of HTBAC on the Blue Waters and Titan supercomputers. We conclude
% with a discussion of the impact of HTBAC, implications for binding affinity
% calculations and near-term future work.


==> related_work.tex <==
\jhanote{A section with a single subsection is bad style. I think this can be
compressed and the need for a subsection removed. See related\_work2.tex}

The strength of drug binding is determined by a thermodynamic property known
as the binding free energy (or binding affinity). One promising technology for
estimating binding free energies and the influence of protein and ligand
composition upon them is molecular dynamics (MD) ~\cite{Karplus2005}. A
diversity of methodologies have been developed to calculate binding affinities
MD sampling~\cite{Mobley2012} and blind tests show that many have considerable
predictive potential~\cite{Mey2017, Yin2017}. We have designed two protocols
with the demands of clinical decision support and drug design applications in
mind: ESMACS (enhanced sampling of molecular dynamics with approximation of
continuum solvent)~\cite{Wan2017brd4} and TIES (thermodynamic integration with
enhanced sampling)~\cite{Bhati2017}. The former protocol is based on variants
of the molecular mechanics Poisson-Boltzmann surface area (MMPBSA), which is
an `approximate' end-point method~\cite{Massova1999}. The latter on the
rigorous `alchemical' thermodynamic integration (TI)
approach~\cite{Straatsma1988}.

Using these protocols, we have demonstrated the lack of reproducibility of
individual simulations for a variety of protein systems, with calculations for
the same protein-ligand combination using almost identical initial conditions
producing widely varying results (binding affinities varying by up to 12 kcal
mol $^{-1}$ for small molecules, whilst flexible ligands can vary even
more)~\cite{Wan2015, Sadiq2010, Wright2014}. Indeed, our work has revealed how
completely unreliable single simulation based approaches are. However, we have
shown that averaging across multiple runs can reliably produce results in
agreement with previously published experimental findings~\cite{Sadiq2010,
Wan2011, Wright2014, Bhati2017, Wan2017brd4, Wan2017trk}, and correctly
predicted the results of experimental studies performed by colleagues in
collaboration~\cite{Bunney2015}. We term this approach ensemble molecular
dynamics, ``ensemble'' here referring to the set of individual (replica)
simulations conducted for the same physical system. In this Section we discuss
the advantages to this approach.

% ---------------------------------------------------------------------------
\subsection{Ensemble Molecular Dynamics Simulations}

Atomistically detailed models of the drug and target protein can be used as the
starting point for MD simulations to study the influence of changes in 
either drug or protein composition on drug binding. 
The chemistry of the system is encoded in what is known as a potential
~\cite{Karplus2002}. 
In the parameterization of the models, each atom is assigned a mass and a charge,
with the chemical bonds between them modeled as springs with varying
stiffness.
Newtonian mechanics is then used to follow the dynamics of the protein and drug and, 
using the principles of statistical mechanics, estimates of thermodynamic properties 
obtained from simulations of single particles.

The potentials used in the simulations are completely under the control of
the user. 
This allows the user to manipulate the system in ways which would
not be possible in experiments. 
A particularly powerful example of this are
the so called ``alchemical'' simulations in which the potential used in the
simulation changes, from representing a particular starting system into one 
describing a related target system during execution. 
This allows for the calculation of free energy differences between the two 
systems, such as those induced by a protein mutation.

MD simulations can reveal how interactions change as a result of chemical alterations,
and account for the molecular basis of drug efficacy. 
This understanding can form the basis for structure-based drug design as well as helping 
to target existing therapies based on protein sequence. 
However, correctly capturing the system behavior poses at least two major 
challenges: The approximations made in the potential must be accurate enough representations 
of the real system chemistry; and sufficient sampling of phase space is also required.
Our previous work demonstrated \cite{Sadiq2010, Wan2011} that running multiple 
MD simulations based on the same system and varying only in initial velocities
offers a highly efficient method of obtaining accurate and reproducible
estimates of the binding affinity.
While the accuracy of force fields could be a source of error, we know from our work to 
date that the very large fluctuations in trajectory-based calculations account for the lion’s 
share of the variance (hence also uncertainty) of the results.

In order for MD simulations to attain widespread use in industrial (and potentially 
clincal) settings, it is necessary that results can be obtained in a timely fashion.
This typically means that results are required in a mattre of days (or at most a week) 
in order that the results can feed into decision making processes.
The necessity for rapid turn around times places additional demands on
simulation protocols which need to be optimized to gain results with a short
turn around time. 
Further to the scientific and practical considerations
outlined above, it is vital that reliable uncertainty estimates are
provided alongside all quantitative results for simulations to provide
actionable predictions.

We have developed a number of free energy calculation protocols based on the
use of ensemble molecular dynamics simulations with the aim of meeting these
requirements~\cite{Sadiq2008, Sadiq2010, Wan2017brd4, Wan2017trk}.
Basing these computations on the direct calculation of ensemble averages facilitates
the determination of statistically meaningful results along with complete
control of errors. 
As we scale up to larger datasets the use of the ensemble approaches will increasingly 
necessitate the use of middleware to  provide reliable coordination and distribution 
mechanisms with low performance overheads.


==> results.tex <==
\subsection{Scaling and Performance Characterization}

We first characterize the overheads of HTBAC and the runtime system. HTBAC
enables concurrent execution of multiple protocol instances. With each new
protocol instance generated for an application, the HTBAC overhead grows to
match the additional requirement of generating and coordinating protocols.

In order to understand the contribution of the various events in HTBAC, termed
as HTBAC overhead, to the total time to completion (TTC) we construct the
following: $TTC = TTX + T_{O}$ where
 \(TTX\) measures the execution duration across all task, including file
 staging, MD kernel execution, and post-executables, and $T_{O}$ the total
overhead is given by the sum of the constituent overheads: $$T_{O} =
T_{O}\textsuperscript{HTBAC} + T_{O}\textsuperscript{EnTK} +
T_{O}\textsuperscript{RP}$$


% \(Time-to-run =
% T(overhead\textsubscript{HTBAC} +
% T(overhead\textsubscript{entk}) +
% T(overhead\textsubscript{rp}) + T(execution)\).

% We define \(T(execution)\) as \(TTX = TTC - T_q\) where \(TTC\) is
% time-to-completion and \(T_q\) is time spent queuing on the HPC machine.



% T(overhead\textsubscript{HTBAC} +
% T(overhead\textsubscript{entk}) +
% T(overhead\textsubscript{rp}) + T(execution)\).

% We define \(T(execution)\) as \(TTX = TTC - T_q\) where \(TTC\) is
% time-to-completion and \(T_q\) is time spent queuing on the HPC machine.


\subsubsection{Weak Scaling Experiments}

Here we show homogeneous and heterogeneous weak scalability of the ESMACS 
and TIES protocols by growing the number of protocol instances while adhering 
to the required number of pipelines. By design of each protocol, an 
increase in the number of instances simply means an increase in the number of 
pipelines. The first weak scalability experiment demonstrates the 
behavior of HTBAC, EnTK and RP using the multiple instances
of the TIES protocols. The second experiment repeats the same design yet replaces
TIES with ESMACS. The third experiment demonstrates concurrent execution of TIES
and ESMACS in the same run. By design of weak scaling, the ratio between the 
number of pipelines and cores are kept constant. As the number of cores 
(measure of resource) changes by a factor of 2, we introduce twice as many 
protocol instances. As designed, the weak scaling property provides insight 
into the size of the workload that can be investigated in a given amount of time.

The HTBAC overhead accounts for approximately 0.1\% of \(TTX\). The remaining
overheads, mainly EnTK and RP, depend on the number of tasks that need to be
translated in-memory from a Python object to a compute unit (CU) description.
As such, it is expected to grow proportionally to the number of tasks. EnTK
submits CU descriptions to a MongoDB used by RP, and the RP pilot pulls these
descriptions from the same database. This pull operation occurs over a wide
area networks, which introduces varying amounts of latency. In addition, each
Stage constructed by EnTK maintains sequential barriers. As such, RP remains
dormant until completion of the current Stage before executing later stages.
The impact of the barrier increases with number of CUs as seen in the 16
protocol instances data point in \ref{fig:weak_scaling}. Together, these two
factors introduce delays in the scheduling of the CUs and results in higher
overheads. Each additional protocol instance contributes to roughly 55
additional seconds in \(TTX\).



% \(TTX\) measures the execution duration across all task, including file staging, MD kernel execution,
%  and post-executables.





%We previously demonstrated weak scaling of the ESMACS protocol in [ref SC] where we showed that a single ESMACS instance could run up to 128 concurrent pipelines.
%\jhanote{1 sentence about how pipelines in ESMACS were simpler than TIES? else the
%reader will say: you did 128 pipelines already... why should I be impressed by a
%small number of pipelines. Important to highlight that the scalability is over
%PROTOCOL INSTANCES and not pipeline instances.} \jdnote{added blurb in
%design \& implementation, removed it from here}

%\subsection{Weak/Strong Scaling Performance Results}

% Therefore our previous ESMACS experiments~\cite{} \jhanote{fix please}
% demonstrates the scalability of ESMACS as a growth in the number of pipelines.



% The goal is to isolate and understand the impact of
% increasing the number of instances, thereby the execution workload.



%The next weak scalability experiment replicates the design of the first experiment using a combination of TIES and ESMACS instances. The comparison of experiment 1 and 2 shows the ability to execute procotols with different resource requirements using one pilot.

\subsubsection {Strong Scaling Experiments}

Next we repeat the same design of the weak scalability experiments but examine
performance of strong scaling when fixing the number of pipelines and varying
the resources. The comparison between weak and strong scalability demonstrates
the overhead introduced by load balancing and scheduling tasks in multiple
generations.



% HTBAC enables concurrent execution of multiple protocol instances.
% With each new protocol instance generated for an
% application, the HTBAC overhead grows to match the additional
% requirement of generating and coordinating protocols. In order
% to understand the contribution of the various events in HTBAC,
% termed as HTBAC overhead, to the total time to run, we construct the following metrics:

% \(Time-to-run = T(overhead\textsubscript{HTBAC} +
% T(overhead\textsubscript{entk}) +
% T(overhead\textsubscript{rp}) + T(execution)\). We define \(T(execution)\) as \(TTX = TTC - T_q\) where \(TTC\) is
% time-to-completion and \(T_q\) is time spent queuing on the HPC machine.

% \jhanote{We should discuss the above. It is difficult to follow..}

% The remaining overheads, mainly EnTK and RP, depend on the number of tasks
% that need to be translated in-memory from a Python object to a compute unit
% (CU) description. As such, it is expected to grow proportionally to the number
% of tasks. EnTK submits CU descriptions to a MongoDB used by RP, and the RP
% pilot pulls these descriptions from the same database. This pull operation
% occurs over a wide area networks, which introduces varying amounts of latency.

% \(TTX\) measures the execution duration across all task, which includes pre-
% executables, the main MD kernel execution, and post-executables.


\subsection{Validation Experiment Results}

To validate the fact that the HTBAC implementation of TIES we 
repeated calculations previously run by Wan \textit{et al.}
\cite{Wan2017brd4}. We selected a subset of the protein ligand systems that
were the subject of that study: they are the transforms between ligand 3 and ligands 1, 4,
and 7. We then performed a full simulation on all 3 systems and calculated the
relative binding affinities (see Table~\ref{tab:exp2}) using HTBAC.

The results show that all three $\Delta \Delta$G values are within error 
of the original study, reinforcing the fact that HTBAC has indeed correctly
implemented the complex workflow of TIES.

\begin{table}
  \centering
  \begin{tabular}{l@{\hskip 1in}r@{\hskip 0.2in}r@{\hskip 0.2in}r}
    \toprule
    System & HTBAC & Wan et. al & Experiment \\
    \midrule
    BRD4 \textbf{3 to 1} & \num{0.39 +- 0.10} &   \num{0.41 +- 0.04} &  \num{0.3 +- 0.09} \\
    BRD4 \textbf{3 to 4} & \num{0.02 +- 0.12} &   \num{0.01 +- 0.06} &  \num{0.0 +- 0.13} \\
    BRD4 \textbf{3 to 7} & \num{-0.88 +- 0.17} &  \num{-0.90 +- 0.08} & \num{-1.3 +- 0.11} \\
    \bottomrule
  \end{tabular}

  \caption{Comparison of the calculated binding free energies using HTBAC, from
  the original study by Wan \textit{et. al} and experimental data. The two theoretical
  studies used the same protcol in principle. This experiment proved that HTBAC
  has indeed implemented TIES correctly, as the calculated values are either
  the same or within error bar of the original study. All values are in
  \textbf{kcal mol\textsuperscript{-1}}.}
  \label{tab:exp2}


\end{table}

%------------------------------------------------------------------------------

\subsection{Adaptive Quadrature Experiments Results}

The impact of adaptivity is clearly seen when $\partial U/\partial\lambda$ is plotted through each iteration. 
Figure~\ref{fig:adapt} shows
how the value of $\Delta$G for one of the test systems improves as the
algorithm places more lambda windows. 

%It is imporant to note, that the new
%points are decided {\it a priori} for reasons discussed above but this is
%opaque to the algorithm. 
This is a proof that we have the adaptive capabilities
and which pave the way for more advanced biosimulation algorithms.

\begin{figure}
\begin{tikzpicture}
\begin{axis}[
  xlabel=$\lambda$,
  ylabel=$\frac{dU}{d\lambda}$,
  xmin=0,
  xmax=1,
  legend pos=outer north east,
  grid=both,
  ]
  \addplot+[name path=alch_1, mark size=1pt, mark=*, color=blue] table [x=lambda, y=p1v]{alch_1.csv};
  \addlegendentry{Iteration 1: inital lambda spacing};

  \addplot+[name path=alch_2, mark size=1pt, mark=*, color=red] table [x=lambda, y=p1v]{alch_2.csv};
  \addlegendentry{Iteration 2: Increasing number of lambda values};

  \addplot+[name path=alch_3, mark size=1pt, mark=*, color=brown] table [x=lambda, y=p1v]{alch_3.csv};
  \addlegendentry{Iteration 3: Optimial number of lambda values found};

  \addplot+[name path=alch_4, mark size=1pt, mark=*, color=black] table [x=lambda, y=p1v]{alch_4.csv};
  \addlegendentry{Iteration 4: Refining function values at optimial mesh};

  \addplot[name path=line, draw=none] {0};

  \addplot fill between[
    of = alch_1 and line,
    split,
    every even segment/.style = {pattern color=blue!50, pattern=vertical lines},
    every odd segment/.style = {pattern color=blue!50, pattern=vertical lines},
    soft clip={domain=0:1},
  ];

  \addplot fill between[
    of = alch_2 and line,
    split,
    every even segment/.style = {pattern color=red!50, pattern=horizontal lines},
    every odd segment/.style = {pattern color=red!50, pattern=horizontal lines},
    soft clip={domain=0:1},
  ];

  \addplot fill between[
    of = alch_3 and line,
    split,
    every even segment/.style = {pattern color=brown!50, pattern=north east lines},
    every odd segment/.style = {pattern color=brown!50, pattern=north east lines},
    soft clip={domain=0:1},
  ];

\end{axis}
\end{tikzpicture}
\caption{The adaptive algorithm reevaluates the efficiency of the lambda window
mesh after every \SI{1}{\nano\second} and makes a decision whether to place
more lambda windows inside certain ranges.}
\label{fig:adapt}
\end{figure}


==> sectionIIInotes.tex <==
% Commented section below will go in Section III and Section IV

% -------------------------------------------------------------------------- 
%
% Drug screening typically occurs in two phases. The first phase runs
% simulations of all drug candidates and determines which candidates become
% lead candidates. This phase is performed using less computationally
% intensive protocols such as ESMACS. Once we eliminate poor-binding
% candidates, we begin the second phase of the campaign where we investigate
% lead compounds using computationally more demanding protocols such as TIES.
% During the second phase, the accuracy of each candidate is evaluated. A
% high level of variability exists in the chemical properties across
% candidates. Therefore, the TIES protocols assumes the most general case in
% evaluating the binding free energy accuracy. To maintain generality, the
% TIES protocol requires 13 evenly spaced simulations, captured using a
% sampling parameter references as $\lambda$ windows in Section III. Although
% generality asserts the correct convergence criteria, this approximation of
% $\lambda$ windows induces higher computational costs as a result of
% executing large yet sometimes unnecessary simulations.

% On the other hand, adaptive methods such as the adaptive quadratures
% highlighted Section III, require less sampling and thereby reduce the
% number of simulations, without sacrificing accuracy. Because this method is
% tailored to every candidate, there is no way to understand \textit{a
% priori} the placement of $\lambda$ windows and thereby the total number of
% simulations.

% This requires the ability to instantiate simulations that predicate on
% intermediate results during runtime.

% Define parameters: added simulations means task count adaptivity and task
% attribute adaptivity. The next set (both number of resources) of
% simulations depends on the output properties of the previous simulations.
% When we adapt the number of simulations, the distribution of resources for
% each task within a static pilot will fluctuate.

% Carefully constructed $\lambda$ placement requires that the workflow can be
% adaptable by creating new computational tasks during execution, thereby
% modify the task graph during runtime. In HTBAC, construction of an adaptive
% workflow is predicated upon the workload management system (define) that
% provides expression of adaptive features.

% while communicating those parameters down to the runtime system (define).


% The post-execution properties are captured by the workload management
% system, EnTK.


% We then perform adaptive experiments to show improvements in
% time-to-convergence.

% -------------------------------------------------------------------------- %


% move this to HTBAC Design & Implementation
% -------------------------------------------------------------------------- %
% As discussed earlier, the free energy is calculated numerically using an
% integration algorithm, integrating the function $\partial
% U/\partial\lambda$ evaluated at discrete of $\lambda$. In a non-adaptive
% case these values of $\lambda$are selected a priori, and having no
% knowledge of the function's shape, equally spaced values are the optimal
% option.

% The aim of the general adaptive quadrature algorithm is to minimize the
% number of function evaluations while still estimating the integral under a
% specified error threshold. In our case a function evaluation means the full
% simulation for a given $\lambda$ window, and reducing this means a
% substantial efficiency gain.

% where each stage runs shorter production simulations of 1 nanosecond. We
% initialize $S4.1$ by assigning 3 equally spaced $\lambda$ windows at $0$,
% $0.5$ and $1$. Once the simulations have converged, we run a post-execution
% estimate the error of the free energy along each interval, i.e. $0$ to
% $0.5$ and $0.5$ and $1$. Once each simulation is complete within a stage, a
% decision is made about whether more $\lambda$ windows are required, and, if
% so, where these windows should be placed.

% We start the simulation with 3 equally spaces lambda windows at $0$, $0.5$
% and $1$ and run the three simulation in parallel just until they have
% converged. Then we estimate the error of the free energy along each
% interval (0 to 0.5 and 0.5 to 1) to determine whether a new lambda window
% needs to be placed halfway in between. The we iterate until no more lambda
% windows need to be placed. Now we determined the minimum set of optimally
% placed set of lambda windows. Using this set we start full simulation
% protocols to calculate the free energy of the alchemical transformation.

% -------------------------------------------------------------------------- %
% In the adaptive workflow, we alter the number of $\lambda$ windows being
% simulated over the course of a protocol instance. The position of new
% $\lambda$ windows depends on the estimated error of the integral measured
% between adjacent windows. Increasing the number of $\lambda$ windows in
% regions of rapid change will increase the accuracy of the overall integral
% to a greater degree than an arbitrarily placed window. In order to
% adaptively add lambda windows, we need access to the $\partial
% U/\partial\lambda$ values during runtime. Therefore, we break down the
% single production simulation stage (S4) \mtnote{I would reference the
% figure with the workflow diagram here} from the nonadaptive workflow into
% multiple smaller stages \mtnote{how many?}, each running for 1 ns. Once
% each simulation is complete within a stage, a decision is made about
% whether more $\lambda$ windows are required, and, if so, where these
% windows should be placed.

% We start out the simulation with 5 replicas of \emph{3} \mtnote{why
% emphasis for 3?} equally spaced $\lambda$ windows, and equilibrate them.
% Then we repeatedly execute shorter production simulations followed by an
% analysis phase which determines where to place new lambda windows. This
% procedure is repeated until convergence, at which point all concurrent
% simulation are terminated. We define convergence as the point in the
% production-analysis loop at which a desired error threshold is reached.

% In non-adaptive experiments we run simulations according to the original
% TIES protocol where the MD simulation step runs for the full 4 ns duration.
% In the adaptive experiments, we still adhere to the same TIES protocol,
% however we stop the MD simulation after each ns and allow the adaptive
% quadratures to calculate the SEM. The calculation determines where to place
% additional lambda windows in the next nanosecond duration. Once we reach a
% level of simulation convergence, we can halt simulations for that candidate
% and shift resources over to another candidate whose simulations have not
% yet started. We demonstrate computational efficiency, i.e. given X number
% of core hours, what is the difference between adaptive accuracy and
% nonadaptive accuracy? By extent we can also begin to inference the
% trade-offs between computational resources and accuracy.

% The benefit of running adaptive simulations produces greater fidelity.
% Since the exact placement of lambda windows and by extent the simulations
% are not known a priori, in the non-adaptive scenario, lambda windows are
% approximated, 13 evenly spaced positions. While this placement does produce
% statistical convergence, it does so at the cost of additional resources.
% Instead, in the adaptive scenario, we begin the MD simulation with 3
% approximated and evenly spaced lambda windows. We run the MD simulation for
% only 1 nanosecond, and aggregate the outputs from those lambda windows in
% order to calculate the RMSE which determines where to position additional
% lambda windows. Since this variability of lambda windows is highly
% dependent on the physical system, the only way to capture more accurate
% placement of lambda windows is during runtime in order to inference lambda
% windows based on intermediate results.

% We can glean two points from this:

% 1) We can stop the simulation once we reach an acceptable error threshold
% 2) To produce tighter binding affinity as some clinical insights may
%    require, given the same amount of core hours, what is the added benefit
%    of running adaptive experiments over nonadaptive, i.e. how much more
%    accuracy do we gain by running adaptive simulations?

